Towards Explainable Evaluation Metrics for Natural Language Generation

Unlike classical lexical overlap metrics such as BLEU, most current evaluation metrics (such as BERTScore or MoverScore) are based on black-box language models such as BERT or XLM-R. They often achieve strong correlations with human judgments, but recent research indicates that the lower-quality classical metrics remain dominant, one of the potential reasons being that their decision processes are transparent. To foster more widespread acceptance of the novel high-quality metrics, explainability thus becomes crucial. In this concept paper, we identify key properties and propose key goals of explainable machine translation evaluation metrics. We also provide a synthesizing overview over recent approaches for explainable machine translation metrics and discuss how they relate to those goals and properties. Further, we conduct own novel experiments, which (among others) find that current adversarial NLP techniques are unsuitable for automatically identifying limitations of high-quality black-box evaluation metrics, as they are not meaning-preserving. Finally, we provide a vision of future approaches to explainable evaluation metrics and their evaluation. We hope that our work can help catalyze and guide future research on explainable evaluation metrics and, mediately, also contribute to better and more transparent text generation systems.

==> abstract_old.tex <==
Unlike classical lexical overlap metrics such as BLEU, most current 
%machine translation 
%high-quality 
evaluation metrics are based on black-box language models such as BERT or XLM-R. %This sets them apart from early metrics based on lexical overlap, as a semantic understanding of language can be encoded. 
% \CL{@Piyawat, with your comment "across systems.in order to ... / for being capable of ..." do you mean "In order to achieve strong correlations to human judgments, their decision processes are difficult to comprehend"? \\--> PL: I meant it may be a good idea to provide a background why people are moving to these pre-trained LMs for metrics. (e.g., to capture nuance in semantics beyond n-gram overlapping.) \\ --> CL: I see, I included a respective sentence above.} 
They often achieve strong correlations with human judgments, but recent research indicates that %they are %[underemployed], 
the lower-quality 
classical %lexical overlap 
metrics remain dominant, 
one of the potential reasons being that their decision processes are %opaque. 
transparent. 
To foster more widespread acceptance of the novel high-quality metrics, explainability thus becomes crucial. 
%Furthermore, explainability techniques that help unveil the internal workings of the metrics need to consider their specific properties, such as: (usually) having continuous output scores and comparing multiple textual inputs. 
In this concept paper, we identify key properties and %(following previous work) 
propose %as well as their impact on how explanations for metrics are evaluated. 
%In addition, 
%Following previous work, which has shown that various goals are pursued throughout the explainability literature, we propose 
key goals %of %explainable machine translation metrics.
of \emph{explainable machine translation evaluation metrics}. 
%e.g., 
%These include to 
%% \PL{Can we rearrange the order here? 1 seems to match 3 whereas 2 matches 4. \\--> As Marina proposed, I would order them by importance \\--> PL: OK}
%(i) identify weak spots, aimed at improving the metrics, (ii) increase  researcher’s trust, and (iii) %%increasing 
%increase the usability for non-experts.   %and 4.) detecting social biases. 
We also %identify and summarize 
provide a synthesizing overview over recent approaches for explainable machine translation metrics and discuss how they %take these properties into account.
relate to those goals and properties. Further, we  conduct own novel experiments, which (among others) find that current %automatic 
adversarial NLP techniques are unsuitable for automatically identifying limitations of high-quality black-box evaluation metrics, as they are not meaning-preserving. Finally, we provide a vision of future approaches to explainable evaluation metrics and their evaluation.  
%Since we find that most of them consider numeric explanation types, we further experiment with designs for textual explanations to complement them. 
%Based on these goals, we give recommendations on which of the approaches are the most suitable selections to solve them %\CL{ToDo: If we give recommendations, we should mention them here (as decribed a comment by Piyawat)}. 
We hope that our work can %provide guidance for 
%guide future research on explainable evaluation metrics,  %and with that, better machine translation models.
help catalyze and guide future research on explainable evaluation metrics and,  mediately, also contribute to better and more transparent text generation systems. 

==> background/ShortSummaryOfTechniques.tex <==
Here we summarize each technique in only 1-2 sentences in order to have an overview for us. Likewise, we write 1-2 sentences on the critique or where we would recommend it. This is written down to improve the current structure of the taxonomy.

Eval4NLP Submissions:
Currently, they are all summarized as one technique, which probably doesn't make much sense, as we compare it with single techniques. Also it would give our paper more techniques to actually compare.

- Word Level Supervision

- Common Techniques (Attention, Additive Feature Attribution) --> kind of difficult to name this. Alternatively we could just list every paper.

- Attention + Metric Embeddings

- Token Matching

==> legacy/legacy_parts_17.01.tex <==
%%% 2

% Todo: remove other current section on this topic
%A main difficulty of Machine Translation is to evaluate the quality of the hypothesis. For most sentences it is possible to produce another sentence conveying the same meaning in an equally natural way. And if multiple sentences are produced, the meaning of a single sentence could be spread.

%Machine translations can be evaluated with machine translation evaluation (MTE) metrics. 
%To give an overview of the characteristics of %these 
%evaluation metrics (for MT), we summarize the main dimensions along which the techniques used in this area can be ordered and differentiated.

%\citet{van-der-lee-2019} describe that natural language is a human construct and therefore the correctness of a translation can be best graded by human experts. However, they also note that this 
Human evaluation is often still considered the gold-standard \citep{van-der-lee-2019},  %kind of evaluation 
but is expensive and slow. 
%Especially, when training a new system for MT, feedback for a generated translation must be given for each output, which quickly becomes infeasible when thousands of samples should be graded every minute. Therefore, human evaluation is mostly used to assess the quality of MT systems after training and as a base to construct and evaluate automated metrics. The other dimensions described below only apply to automated metrics.

%This is done under the assumption that it is not easy to check for a human, whether a model is just using phrases it has already seen during training or if it generates text more freely.

%Embeddings are vector representations of textual or symbolic inputs. 
%Methods that learn


%A word such as ``bass'', which could be a sea bass or an instrument, would receive the same vector representation. Further, they summarized that embeddings like one-hot-encodings are used to present tokens as numbers, which enables mathematical operations. 
%Dimensionality-reduced embeddings additionally would allow to encode properties such as \textit{meaning} into the vector representations. 
%Thereby, textual units can be compared by %distance metrics. In one-hot encoding, all words have the same relation, e.g. a fish is as similar to a whale as to an elephant. 
%In dense representations such as Word2Vec \citep{mikolov-2013} or GloVe \citep{pennington-2014} a word like `fish' might lie closer to the whale. 

%Depending on the context surrounding a token, these representations can differ between words such as ``bass'', that can have a different meaning in different contexts. 
%Additionally, they allow to find words that are close to each other in a specific context. This type of embedding is usually achieved by leveraging the hidden states of a transformer model after a forward pass of the tokens that should be encoded. 
%In MTE, this allows to compare the meaning of sentences rather than whether their words have similar meanings in general. 

%\citep{zhang-2020}. %Thus, this technique requires preceding human effort to generate ground truth translations and is more expensive. Additionally, this kind of 
% References can be seen as a form of supervision.

%When multilingual embeddings are trained, there is an intuition that words with similar context in different languages should be close to each other. 
%This is leveraged by using distance measures \citep{zhang-2020,zhao-2020} on these embeddings or by directly learning to predict human-like scores \citep{sellam-2020}. 

%\item\textbf{Combining source and reference sentences:} The recent metric COMET \citep{rei-2020} combines the usage of source and reference sentences to achieve a better correlation with human judgements in predicting the score of the hypothesis.

%This is fitting for metrics such as BLEU or METEOR that do not use learned representations of words or sentences. 

%\citep{ranasinghe-etal-2020-transquest-wmt2020}
%\CL{there is already a source for the transquest paper, which I change to here. Does it make a difference if we cite their Coling or their WMT paper? I think the coling one has a little more detail. SE: Ok}. 

%It is to note 
%We note that \citet{yuan-2021} only feature the reference-based case in their description of the dimensions ``Unsupervised Matching'' and ``Supervised Regression''. With e.g. BERTScore \citep{zhang-2020} with multilingual embeddings \citep{song-2021} for ``Unsupervised Matching'' or MonoTransquest \citep{ranasinghe-2020} for ``Supervised Regression'' this dimension also applies to the reference-free dimension.

%Segment-level evaluation compares scores that are assigned on the level of one or multiple sentences and system-level evaluation compares estimates on how good translation systems are performing \citep{mathur-2020}.\todo{SE: system-level evaluation compares metric scores on system-level to human scores on system-level? --> yes (their averages). You are right, this is redundant. Here maybe we ould only mention doc and word level.} Another option is evaluation on a document-level \citep{mathur-2020}.\todo{SE: system- and segment-level have been introduced before, maybe reduce redundancy}

%%% 3

% On the other hand, we use the term \textit{interpretable} if the model can be passively understood.

% \todo{SE: I made the below a footnote as I'm not sure about its importance --> ok :), though the current document error is occuring here, just to keep it in mind\\--> PL: I decided to comment this footnote out as I will touch upon this point in the main content.} 
% \footnote{These definitions are similar to the concepts of model transparency and post-hoc interpretability described by \citet{lipton-2016}. There is, however, an important difference in our terminology that the model itself can provide explanations, too.
% % \todo{SE: in our terminology? --> yes} 
% Lipton would count this type of explanations towards model transparency; however, it does not necessarily lead to interpretability in the above sense. For example, in the Eval4NLP 2021 shared task \citep{fomicheva-2021}, word-level scores are used to explain sentence-level metrics (see section \ref{eval4nlp}). Thereby, the word-level scores can be extracted with post-hoc explainability techniques %, e.g. with 
% such as LIME \citep{ribeiro-2016} 
% %or Integrated Gradients \citep{sundararajan-2017} 
% as \textit{Explanators}. On the other hand, a metric could inherently produce word-level scores together with sentence-level scores. Such metrics are explainable, as their more verbose output provides explanations for the sentence level. Still, they are not necessarily interpretable, as potentially underlying language models cannot be passively understood, e.g. by a human inspecting their parameters. In contrast, we consider metrics like BLEU as interpretable, as their full process can be understood by an audience with a reasonable background in computer science.}  


%Based on recent surveys, we identify the following distinctions: \PL{It is important to define interpretability and explainability, but the whole set of bullet points here may be too far away from MT. --> yes, for now I comment the other points out}
%\begin{itemize}
%    \item \textbf{No differentiation}: The term \textit{explainability} is relatively new, while \textit{interpretability} has been used for a longer time \citep{adadi-2018, abdul-2018, barredo-arrieta-2020}. Due to this reason, most earlier works use the term \textit{interpretability} \citep[e.g.][]{lipton-2016, ribeiro-2016, li-2017}. Some newer works explicitly state that they use the two terms interchangeably \citep{adadi-2018, carvalho-2019, miller-2019, jacovi-2020}. Other works that do not make a distinction are \citet{biran-2017, xu-2019, bhatt-2020, vassiliades-2021}. 
%    \item \textbf{Explainability as umbrella concept}:  \citet{gunning-2017} present interpretable models as a subcategory of explainability. Likewise, \citet{doran-2017} define explainability as umbrella concept of \textit{comprehensibility} and \textit{interpretability}, where comprehensibility is the degree to which a model can generally be reasoned about by a human and interpretability describes that the mapping function between input and output can be understood in detail. 
%    \item \textbf{Interpretability as precondition for explainabilty}: \citet{montavon-2018, gilpin-2019} describe interpretability as a precondition to explainability. The interpretability definition of \citet{gilpin-2019} equates interpretability with the concept of \textit{plausibility}

% \PL{I think it's more like \textit{understandability} rather than \textit{plausibility} in their work. -->    I think understandability is another problematic term which itself is also not clear. Gilpin et al say "for a system to be interpretable, it must produce descriptions that are simple enough for a person to  understand using a vocabulary that is meaningful to the user." Plausibility is the capability to give explanations that appeal to humans (e.g. in jacovi's paper), i.e. sound reasonable to a user, even if not correct. To me this definition sounds pretty similar.
% \\ --> PL: To me, both are clearly different. People can understand what the explanation says though they do not agree with it. In this case, the explanation is understandable but not plausible.\\ --> CL: Ah thanks, yes now I see the difference. For completeness below (where i also commented the comment out) I think they are more similar.}

%, which we describe later in this section. Further, they define \textit{completeness} as a further requirement for explainability, which equates the concept of %\textit{faithfulness}\PL{Also, not sure if it is equivalent to faithfulness in their work. --> Here Gilpin say "The goal of completeness is to describe the operation of a system in an accurate way." From my point of view this mostly matches the faithfulness definition of for example Jacovi}. \citet{montavon-2018} take a different approach and describe interpretations as the mapping from an abstract domain (e.g. a neural network's weights) to an interpretable domain (e.g. words). Then, an explanation would highlight important details in the interpretable domain (e.g. which words are important).
%    \item \textbf{Passive Interpretability, Active Explainability}: Some works use the two terms to distinguish the notion of whether a model's process, e.g. the algorithm or the role of parameters, can be passively understood, or whether explanations are actively generated that do not necessarily provide a direct insight. \citet{barredo-arrieta-2020} use this distinction and define interpretability as a synonym of transparency, i.e. how much introspection the model offers by passively looking at it. Based on an English dictionary entry, they define explainability as an active process ``to make something clear to understand'' that is targeted towards an audience. \citet{burkart-2021} note that a common definition would be that interpretability has the goal of understanding a model as a whole, while explainability describes the means of providing explanations on it, even if it is a black box. However, throughout their paper the terms are used interchangeably. \citet{bodria-2021} also define explainability as the capability to actively generate valid explanations for a model's behaviour, while interpretability is the capability of passively understanding a model's behavior. \citet{israelsen-2017} also use such a distinction.
%\end{itemize}

%These viewpoints are illustrated in figure \ref{fig:InterprExpl}. In this survey, we follow the fourth viewpoint. I.e., we follow \citet{barredo-arrieta-2020} and view a model as explainable, if the model or some external instance (described as \textit{Explanator} in the figure) can actively provide explanations that make the decision process or the output more clear to a certain audience. On the other hand, we use the term \textit{interpretable}, if the model can be passively understood. These definitions are similar to the concepts of model transparency and post-hoc interpretability described by \citet{lipton-2016}. There is, however, an important difference in that the model itself can provide explanations, too. Lipton would count this type of explanations towards model transparency; however, it does not necessarily lead to interpretability as in the above definition. For example, in the Eval4NLP 2021 shared task \citep{fomicheva-2021}, word-level scores are used to explain sentence-level metrics (see section \ref{eval4nlp}). Thereby, the word-level scores can be extracted with post-hoc explainability techniques, e.g. with LIME \citep{ribeiro-2016} or Integrated Gradients \citep{sundararajan-2017} as \textit{Explanators}. On the other hand, a metric could inherently produce word-level scores together with sentence-level scores. Such metrics are explainable, as their more verbose output provides explanations for the sentence level. Still, they are not necessarily interpretable, as potentially underlying language models cannot be passively understood, e.g. by a human inspecting their parameters. In contrast, we consider metrics like BLEU as interpretable, as their full process can be understood by an audience with a reasonable background in computer science. 

%\begin{figure}[!tbp]
%  \begin{subfigure}[b]{0.49\textwidth}
%    \includegraphics[width=\textwidth]{images/IvE1.png}
%    \caption{No Differentiation}
%    \label{fig:InterprExpla}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[b]{0.49\textwidth}
%    \includegraphics[width=\textwidth]{images/IvE25.png}
%    \caption{Explainability as umbrella concept}
%    \label{fig:InterprExplb}
%  \end{subfigure}\\
%  \begin{subfigure}[b]{0.49\textwidth}
%  \centering
%    \includegraphics[width=0.7\textwidth]{images/IvE3.png}
%    \caption{Explainability as a step up from interpretability}
%    \label{fig:InterprExplc}
 % \end{subfigure}
  %\hfill
%  \begin{subfigure}[b]{0.49\textwidth}
%    \includegraphics[width=\textwidth]{images/explainability_interpretability.png}
%    \caption{Passive Interpretability, Active Explainability}
%    \label{fig:InterprExpld}
%  \end{subfigure}
%  \caption{Viewpoints on Explainability and Interpretability}
%  \label{fig:InterprExpl}
%\end{figure}

\iffalse
\CL{todo: drop or shorten}
%Like explainability techniques themselves, their evaluation is challenging. 
Evaluation of explainability techniques is challenging. 
As explanations can target different goals, evaluation setups might not fit across all tasks. A common requirement is that a technique fulfills the properties of \textit{Faithfulness} and \textit{Plausbility} \citep{jacovi-2020}. %The first 
Faithfulness 
refers to the technique's capability of accurately explaining a model (in our case a metric).\todo{SE: maybe remove the metric case here?} Plausibility on the other hand refers to the capability to give explanations that appeal to humans. It is important that both of them are fulfilled to some degree, which is emphasized by the example in Figure \ref{fig:PlausibilityIssue}. An explainability technique that only fulfills plausibility does not necessarily add information about a metric, or why it returned a certain score. I.e. the technique could even provide results contradicting to the metric's output and be plausible. While these ``explanations'' might still have desired properties, they do not fulfill the definition of explainability and the explainabilty technique itself might be used as separate metric. An explainability technique that only fulfills faithfulness does not improve the understanding of the explained metric\PL{It helps us understand that the metric works irrationally though. --> I am not sure. Lets say you explain BLEURT by presenting BLEURT itself as an explanation. Then this is faithful, as BLEURT itself faithfully represents BLEURT. Still, this explanation does not improve on our understanding of whether BLEURT works or not. I guess you could say that evaluating that "explanation", which is BLEURT itself, with correlation to human scores gives you a better understanding. Though I am not sure I'd count that towards explainability.
\\ --> PL: It's not clear to me why you can use BLEURT itself as an explanation given that BLEURT is based on a black-box model BERT. Also, what does it mean by ``better understanding'' in your second last sentence? It is the better understanding of what?  
\\ --> CL: I think this notion could be explained with the LIME paper, where they say "Although it is often impossible for an explanation to be completely faithful unless it is the complete description of the model itself [...]". They define explanations as models g of a class of potentially interpretable models G and constrain their complexity using a complexity measure Omega(g) such that the explanation is understandable. Thereby, g takes a binary input that indicates feature absence or presence. So what I meant here is that, if you only need a faithful explanation you don't have to care about Omega(g) and just look for a g that is as close to the original model as possible (potentially one that returns the same output in all cases). Without LIME's restriction to binary features, the closest model would be the model itself. \\
Now, assuming the model could be seen as an explanation of itself (that is not plausible/understandable), then you could probably interpret that you still get some knowledge/understanding from that, as you could do standard evaluations such as checking correlation to human annotations. But I would not write that second thing, as there is probably no reason to phrase it like this. \\
Another paper that would support this notion is the SHAP paper: "The best explanation of a simple model is the model itself; it perfectly represents itself and is easy to understand. For complex models, such as ensemble methods or deep networks, we cannot use the original model as its own best explanation because it is not easy to understand." I.e. we wouldn't understand it, but it would be faithfully represented. \\
I guess the question here is, whether understandability is a precondition to both faithfulness and plausibility, or only to plausibility (or even to plausibility. I guess something might be plausible without me understanding it?).
}, as the explanation does not appeal to humans. For example, the metric \textit{word-level Transquest} \citep{ranasinghe-2021} could be seen as plausible explainability technique for the metric \textit{BLEURT} \citep{sellam-2020} (if the source is available). Likewise, BLEURT could be seen as a faithful explanation of itself \citep{ribeiro-2016}. Previous taxonomies suggest that plausibility evaluation involves humans, while faithfulness evaluation applies metrics without human judgment \citep{deyoung-2020}. This is supported by \citep{jacovi-2020} who hypothesize that it is not possible to grade faithfulness when human judgments are involved. We highlight a number of evaluation approaches that were introduced to measure each of the properties.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{images/PlausibilityIssue.png}
    \caption{An example highlighting a shortcoming of plausibility. An explainability technique might generate plausible explanations, even when the model's output is incorrect.} \label{fig:PlausibilityIssue}
\end{figure}

%\subsubsection{Plausibility}
\paragraph{Plausibility}
\label{Plausibility}
Evaluation methods for plausibility need to consider how well explanations can be understood by a human audience. Therefore, plausibility evaluation involves human judgments. 
\citet{Lertvittayakumjorn-2019} design multiple human evaluation experiments, two of which tackle plausibility:
\begin{itemize}
    \item \textbf{Justify an explanation:} They select samples for which a well-trained model has a high classification confidence. Then they explain outputs of the model with an explainability technique. By only presenting the most important features in the explanation, a human should predict the output of the model. 
    \item \textbf{Help humans decide in uncertain situations:} They select samples, for which a well-trained model has a low classification confidence. Then they explain them using an explainability technique. By presenting the most important and most negatively important features, as well as the model's output, a human should predict, whether a model is correct.
\end{itemize}
Due to the numeric output of MT evaluation metrics, these approaches are problematic, as other measurements of prediction confidence would need to be employed. Still, the evaluation of how explanations support human work \citep{doshi-velez-2017} is a paradigm that could be used for metrics with numeric output as well. For example, future work could consider to apply the notion of simulatabilty\PL{Is it really about plausibility? --> Hm, right it is probably a mix of both that would be evaluated with this. If explanations are not faithful, simulation would not be possible. If they are not plausible, humans could not understand them and not simulate well. Problematic would be to which degree each of them is involved. I.e., does weak simulatability mean weak plausibility or faithfulness. So maybe we shouldn't list this as an idea for the future. Or should find an improvement.
\\ --> PL: To me, simulatability measures understandability (not plausibility) + faithfulness. \\ --> CL: I think I would have seen understandability as an umbrella term for explainability and interpretability. As both of them would enable me to understand my model better. Explainability could (potentially) be measured in terms of plausibility and faithfulness. So, if we can define it like that, I'd say you get an explainable model, if your explanations are both faithful and plausible and this would therefore also make it understandable. In your previous comment you said that humans can also understand explanations if they do not agree with them. I think here the term understand is somewhat underspecified (explanation understandability vs model understandability). I.e. "I can understand what it is explaining to me, but I cannot understand why it is giving the explanation for this model, as I don't agree with it". Therefore, the explanation might be understandable, but not the model itself, when I don't get plausible explanations. \\
Summary: I think it would measure model understandability which originates from the other two concepts.
} \citep{lipton-2016} to evaluate the plausibility of metrics. Concretely, we could follow the approach by \citep{hase-2020}. In case of MT metrics, this approach would evaluate, how close participants of the evaluation can predict the score of a metric before and after receiving an additional explanation.

Rather than evaluating how explanations support humans in their task execution, other works evaluate the correlation to pre-annotated human explanations. \citet{fomicheva-2021b} follow this setting in machine translation evaluation and introduce a dataset with human-annotated rationales, which they use to compute the correlation with feature-importance explanations. Thereby, due to the alignment with human judgment, explainability techniques that generate explanations with a high correlation have a high plausibility (this dataset is described in more detail in section \ref{eval4nlpdata}).


%\subsubsection
\paragraph{Faithfulness}
\label{Faithfulness}
As advocated by \citet{jacovi-2020}, most evaluation methods for faithfulness do not incorporate human judgments.\todo{SE: these authors say not to use human judgments. Why? --> They had a thought experiment showing that humans cannot grade this diretly} The following are common techniques used throughout the literature:
\begin{itemize}
    \item \textbf{AOPC}: The area over the perturbation curve (AOPC) score is a metric introduced by \citet{samek-2017} in the domain of computer vision. It is computed as follows:
    $$\textit{AOPC}=\frac{1}{L+1}(\sum_{k=0}^Lf(x_{\textit{MoRF}}^{0})-f(x_{\textit{MoRF}}^{k}))_{p(x)}$$
    $$x_{\textit{MoRF}}^{0}=x$$
    $$\forall 1\leq k\leq L:\;x_{\textit{MoRF}}^{k}=g(x_{\textit{MoRF}}^{k-1},r_k)$$
    In relation to MT metrics, $f$ is the metric function. $x_{\textit{MoRF}}^{k}$ is the original hypothesis with $k$ removed tokens. The tokens are removed in order of their feature-importance (MoRF means ``most relevant first''). The position of the next token is given by $r_k$ and the function $g$ handles the replacement or removal. The intuition behind this evaluation method is that the output probability $p(x)$ of a model should drop more if an important feature is removed than when an unimportant feature is removed. Hence, when the input features are removed one by one, based on their importance, the curve of predicted probabilities should first fall strongly and then flatten. Therefore, if the computed area over the curve of perturbation outputs is big, the feature-importance method is said to be faithful. In terms of MT metrics, the curve does not show the drop in predicted probabilities, but the drop in predicted metric scores.\PL{A figure of AOPC curve would be helpful.}\CL{Todo}
    
    A number of variations to this score have been proposed in the literature. \citet{deyoung-2020} don't remove the tokens one by one, but rather replace a certain percentage of most important features in each step (1\%, 5\%, 10\%, 20\%, 50\%). This might capture token dependencies between words, though there might for example also be dependant words of which one is removed in the 1\% step and one in the 5\% step. 
    
    Another variant is proposed by \citet{kim-2020}. $g$ is modified to replace with random likely words predicted by a language model, rather than removing or replacing with a fixed word. They propose this approach in order to prevent out-of-distribution problems when evaluating modified sentences.
    
    A very similar approach is called \textit{degradation tests} \citep{schulz-2020,chen-2021}. These additionally consider the least relevant perturbations and are based on the area between the curves.
     
    \item \textbf{Post-Hoc Accuracy} is a method for classification settings that measures how many of the original class predictions are still correct if only a set number of most relevant tokens is kept in the input \citep{chen-2018}. This could be adapted to metrics with numeric outputs by evaluating, how many of the metric predictions are still within a certain range after only the most relevant tokens are kept.
    
    \item \textbf{Glass-Box approaches}: Another option to measure the faithfulness of an explainability technique is to explain interpretable metrics or metrics that provide explanations themselves \citep[e.g.][]{ribeiro-2016,Decao-2020, fomicheva-2021,leiter-2021}. This provides a ``synthetic ground truth''. However, explaining interpretable metrics such as BLEU might be easier for the explainability techniques than to explain SOTA metrics like BLEURT. Most explainable metrics that provide explanations themselves are stronger than BLEU, but are not necessarily faithful.\PL{If they are not faithful, how can they be used to evaluate faithfulness of another explanation method then? --> I meant that depending on the architecture they might be faithful, but don't have to be. E.g. attention vs word-level bertscore \\ --> PL: But if we want to evaluate another explanation method by comparing their outputs with explanations directly generated from these explainable metrics, we should require faithfulness from the reference explanations, shouldn't we? --> CL: Ah yes I see, it would of course make sense to add this as a condition for this kind of evaluation. I'll add it.} For example, consider a metric that generates an additional text description of a single metric score with respect to an input. If the text generation is learned based on human annotated explanations of human scores, there is no guarantee that the metric actually followed a certain process internally.
\end{itemize}    

Recent work has explored the out-of-distribution (ood) problem that comes with the fixed removal or replacement of inputs to explainability techniques and evaluation methods \citep{kim-2020, rychener-2020}. They consider that neural networks might not have learned how to react to inputs with unusual permuted features, leading to an insincere evaluation. We note that many of the above approaches are prone to this problem. \citet{kim-2020} use mask replacement to keep the perturbed sentences in-domain. However, we note that this introduces another black-box component into the evaluation metric of an explainability technique, which might be dangerous.

Another problem we see is that the explainability evaluation might be biased towards the explainability technique. E.g. if evaluation method and explainability technique both use word removal, they favour each other more than if one of them uses mask replacement. Likewise, an evaluation method that leverages mask replacement might favour explainability techniques that use language models. 
    
Due to these considerations, the evaluation of faithfulness needs further investigation in the future.\todo{YG: you may say it needs more investigation; present it in a more positive tone :)}

%\subsection{Domain specific NLG metric Terminology}
%Some of the works discussed throughout this paper have been applied to subtasks of NLG. In this section. We define terminology that is specific to certain subtasks:
%\begin{itemize}
%    \item \textbf{Reference-Free vs Reference-Based:} These terms are usually used in the context of MT evaluation and could also be applied to other tasks of cross-lingual language generation. A metric is called reference-based, if it requires one or multiple human reference translations to compare with the hypothesis \citep{zhang-2020}. Thus, this technique requires preceding human effort to generate ground truth translations and is therefore more expensive. Additionally this kind of metrics cannot be used in cases where no expert speaking both languages is available. In contrast, \textit{reference-free} metrics do not require a reference translation to grade the hypothesis \citep{zhang-2020,ranasinghe-2020}. Instead, they use the similarity to the source sentence to determine the quality. In the literature, reference-free MT is also referred to as "reference-less" or "quality estimation". The recent MT metric Comet \citep{rei-2020} combines the usage of source and reference to achieve a better correlation with human judgments.

%\end{itemize}
%The surveys by \citet{sai-2020,celikyilmaz-2020} provide a good further overview.
\fi

predictions. 
% Hence, there are two concepts 
% \PL{Overall, should we mention approaches for XAI in general but not yet applicable or impossible in the context of MT evaluation? --> Do you refer to the approaches here, or to the dimensions? As discussed in our meeting, i'd move the dimensions to future work. For the approaches I am not sure, as they might fit nicely into the taxonomy anyways (the ones currently described)\\ --> PL: If approaches mean how to evaluate explanations, what I said above refers to dimensions. And I agree with you that those that haven't been applied to MT eval. could be future work.}
% \subsection{Definition}

%%% 4

%For explainable NLG, we work out the following goals:
%\begin{itemize}
%    \item \textbf{Accessibility} describes the goal of allowing non-experts to use a model by providing insights into it \citep{lipton-2016,barredo-arrieta-2020}.
%    \item \textbf{Confidence} is the goal of providing confidence estimations for a model's output to support further decision making \citep{lipton-2016,barredo-arrieta-2020}.
%    \item \textbf{Causality} describes the goal of using the information gained from a trained model to infer causal relationships \citep{lipton-2016,barredo-arrieta-2020}. This means, a model gives insights into real world correlations, which can then be used to design experiments that test for causality.
%    \item \textbf{Fair \& Ethical Decision Making} describes the goal of ensuring a model to be unbiased and to adhere to laws and regulations by understanding its decision process \citep{lipton-2016,barredo-arrieta-2020}. Explainability can improve fairness by supporting the selection of unbiased models.
%    \item \textbf{Informativeness} describes the goal of increasing the amount of information conveyed by or about a model \citep{lipton-2016,barredo-arrieta-2020}. For example, rather than providing only a probability for a predicted class, or a regression result, additional information such as "the model followed rule X" can provide further support. This can help in supporting decisions that are made based on a model's output. Additionally it can highlight the flaws of a model, so that it can be improved in further development efforts.
%    \item \textbf{Transferability} describes the goal of understanding a model's capability to generalize to unknown domains \citep{lipton-2016,barredo-arrieta-2020}. E.g. \citep{ribeiro-2016} describe an example where a model used the presence of snow to distinguish between wolfs and huskies. By using their technique \textit{LIME} this error became clear, leading to the understanding that the model would not generalize well.
%    \item \textbf{Trust}: \citep{lipton-2016,carvalho-2019,barredo-arrieta-2020} identify trust as an often pursued goal across several research papers. \citep{lipton-2016} states however that trust is a property that is difficult to define. They consider that trust in that a model makes the right decisions might be achieved by having a high accuracy but it might also be achieved by only having a high accuracy in the same situation as a human does. It might also be trusted if it operates well without being biased, e.g. treating some individuals differently to others based on race or gender. Likewise, some individuals might only trust a system following their own biases. Thus, most of the other goals on this list may or may not achieve the subjective property of trust. 
%    \item \textbf{Safety}: \citet{doshi-velez-2017} discuss that end-to-end systems are difficult to fully test. Therefore explanations can provide a measure of a systems safety. 
%    \\For this goal to be fulfilled it is important for the explanations to be \textit{faithful}, as discussed later in this section.
%\end{itemize}
%Besides these, sometimes other goals such as Privacy Awareness (does a model use sensitive information?) and Interactivity (does a model interact with a human?) are considered \citep{barredo-arrieta-2020}. 



==> legacy/old_dimensions.tex <==
\begin{table*}[!htb]
\small 
\centering
\begin{tabularx}{\textwidth}{lXXXXXXX} %{p{4.5cm}ccccccc}
     \toprule
     \textbf{Work} & \textbf{Type} & \textbf{L/G} & \textbf{A/S} & \textbf{Method} & \textbf{Eval} & \textbf{Goals} & \textbf{Specifics}\\ \midrule
     \citet{fomicheva-2021} 
     % ,fomicheva-2021b --- too long for the line
     & FI & L & A+S & Var. & Plaus. \\\midrule
     \citet{chen-2021} & FI & L & A & Pert. & Faithf. \\\midrule
     \citet{yuan-2021} & TBD & L & A & TBD & Plaus. \\\midrule
     Adversarial Attacks & EbE & L & A & Pert. & -\\\midrule
     \citet{kaster-2021} & EbS/CA & G & A & TBD & Faithf.\\\midrule
     \citet{sai-2021} & CA & G & A & Pert. & TBD\\
     \bottomrule
\end{tabularx}
\caption{Explainability for MT metrics. The types are Concept Attribution (CA), Feature Importance (FI), Explanation by Example (EbE) and Explanation by Simplification (EbS). L/G considers Local (L) vs Global (G) and A/S considers Agnostic(A) vs Specific(S). The "Eval" column indicates whether the authors evaluated with respect to plausibility and/or faithfulness. The column ``Goals'' specifies, which of the goals of section \ref{} can be addressed with the respective techniques. Thereby, we consider (B)ias detection, metric (D)iagnosis and metric (E)xpressiveness. Lastly, "Challenges" shows which of the properties \textit{(m)ultilingual input, varying (s)cales, (n)umeric output, relation to translation (e)rrors and interdependent (p)airwise input} are being addressed.}
\label{taxonomy}
\end{table*}

%\citet{lipton-2016} highlights the difficulties in giving a concise definition of interpretability (here also explainability). One of the reasons he names is that there is a diverse set of goals followed throughout the literature. We summarize some of the key properties identified by other surveys:

\subsection{Dimensions of Explainability} \CL{todo:only describe dimensions that occur in the taxonomy table}
\label{sec:dimensions}
Now that we have noted desiderata and properties of explainable MT, we describe dimensions that are used across the literature to describe the properties of explainability techniques. We leverage these dimensions to provide a taxonomy of recent approaches for explainable MT.

\subsubsection{Dimension: Explanation Type}
\label{explanationType}
Based on the previous definitions of interpretability and explainabilty an explanation is additional information that is provided by a model or a separate component in order to make the model's outputs more clear \todo{YG: more clear or clearer? } to a specific target audience. We highlight different types of explanations and discuss their application for MT evaluation:
\begin{itemize}
    \item \textbf{Text Explanations} are explanations in the form of generated texts providing information on a model's output \citep{lipton-2016}. For MT evaluation, such an explanation could be a text such as
    ``The hypothesis received a score of 0.8 as it captures all the facts of the reference, but has grammatical errors for word A and word B''.
    %\item \textbf{Visualizations} are explanations in the form of plots, generated images and other, mostly non-symbolic representations \citep{lipton-2016,adadi-2018}. For MT evaluation, such an explanation could be a plot of dimensionality reduced word embeddings of a hypothesis and a reference, showing the distance in alignment between the two. This would for example help to explain XMoverScore and BERTScore, which are based on the distances of contextual word-embeddings.
    \item \textbf{Explanations by Example} present similar cases (as the current input/output pair) from a database of understood cases \citep{lipton-2016,adadi-2018}. In MT evaluation a score might be explained by presenting examples of hypothesis-reference or hypothesis-source pairs that achieved a similar score (by the same model). However, this leaves the deduction of actual similarities to the user or another model. Explanations by example can be further differentiated into \textit{prototypes, criticism and counterfactuals} \citep{ruping-2006, wachter-2018,adadi-2018, burkart-2021}. Prototypes are similar examples representing one or multiple input-output pairs. They are helpful if the presented example is well-analyzed. If prototypes are pre-computed, criticisms (discriminating samples) are instances that are not represented well by them, i.e. for which no good prototype can be found. Counterfactual explanations describe examples with minimal changes to the input that change the output in a noticeable way (in the case of classification changes the class).
    \item \textbf{Explanation by Simplification} is achieved by training a simpler model to mimic the results of a complex one \citep{barredo-arrieta-2020}. In MT evaluation this would for example be given if it would be possible to represent a BERT model as a decision tree that would then be considered an explanation.
    \item \textbf{Feature Importance/Relevance Explanations}\footnote{\citet{barredo-arrieta-2020} note that these terms are used interchangeably} are explanations that assign a relevance score for every input feature \citep{barredo-arrieta-2020}. For example, given a hypothesis "this is not a cat" and a reference "this is a cat" an explanation of a perfect MT metric should assign a high negative relevance to the word "not". 
    %\item \textbf{Rule Based Explanations} consist of one or more decision rules that allow to predict the behavior of a model if the conditions of the rule are met \citep{adadi-2018}. This is especially useful for classification as it allows to simulate a model's outcome. In the case of MT metrics that return numeric outputs, the scale could be discretized and a rule could for example be ``if phrase A, B and C are present in a hypothesis, the score will be X''. %\citet{danilevsky-2020} refer to rule based approaches as \textit{declarative induction}.
    \item \textbf{Local Explanations:} There is a difference between the scope of local explainability methods and explainability methods that provide local explanations. While local explainability methods (see \ref{localMethods}) explain a model's output for a single input-output pair, a local explanation only applies to the neighbourhood around the input \citep{lipton-2016}. Here, the term neighbourhood is open for choice. \citet{ribeiro-2016} use the proximity of binary feature masks. \todo{YG: an example will help here. what it means by 'neighbourhood around the input'? a sentence similar to the hyp/ref/input sentence? --> CL: I added a sentence}
    \item \textbf{Concept Attributions} describe, to what extent a user provided concept is fulfilled in the data \citep{bodria-2021}. \citet{bodria-2021} state that this type of explanation is used in some approaches in the area of computer vision. In MT evaluation, a user could for example provide categories for \textit{missing facts} or \textit{incorrect sentence structure}.
\end{itemize}
The different explanation types are not fully distinct \todo{orthogonal? --> CL: would this be the better term? I think it would mean more or less the same.}. E.g. \citet{ribeiro-2016} build simplified, linear models, whose weights can be used as local explanations for changes applied to specific input features.\PL{I would see simplification (using surrogate models) as a method. --> CL: So you would place it in another dimension? At one point the output of surrogate model methods is the surrogate model/simplified model, so I'd have placed it in the explanation (output) type section} Therefore, they provide local feature importance explanations by simplification.
\citet{lipton-2016, barredo-arrieta-2020} list the presented explanation types as post-hoc explanations only. Following the definition of explainability given above, in this work, we will also use these explanation types for those that are actively generated by the model itself. 

\subsubsection{Dimension: Local vs Global Explainablity}
\label{localMethods}
Another common distinction used in taxonomies is the one of local vs global explainability techniques \citep[e.g.][]{doshi-velez-2017,arya-2019,carvalho-2019, danilevsky-2020,bodria-2021}. Global techniques try to characterize the behaviour of a model as a whole. In explainable MT, global explanations give insight into the general factors a metric considers when assigning a score (see section \ref{globalExpPaper}).
\todo{YG: it's a bit hard to imagine what a global explanation would be like for MT evaluation. We may need more explanations or discussions here. --> CL: Later in the paper, there are two approaches that are being described. I added references}
Local techniques in contrast, provide explanations of a single input-output combination (see section \ref{localMethods}). For example, given a reference translation "My dog is lovely" and a machine translation "My dog is angry" with a predicted score of 0.7, a local explanation describes why the metric predicted this score for this instance.\\
%\citet{guidotti-2018} further divide this distinction into outcome explanation, model inspection and model explanation. Outcome explanation thereby is synonymous to local explanations. Model explanation techniques are analogous to global techniques and model inspection techniques follow the goal of identifying a model's internal properties without necessarily providing global understanding. As an example \citet{guidotti-2018} refer to the forming of understanding of the role of certain neurons in a neural network through explanations. 

\subsubsection{Dimension: Model Agnostic vs Model Specific}
\label{agnost}
\citet{carvalho-2019, barredo-arrieta-2020, bodria-2021} differentiate between model-agnostic and model-specific techniques. Model-agnostic techniques can be applied to any type of model while model-specific techniques can only be applied to specific types of models. 

%\subsubsection{Dimension: Input Data Type}
%\citet{guidotti-2018,arya-2019,bodria-2021} distinguish explainability techniques based on the datatype the explained model takes as input. They differ between \textit{tabular-}, \textit{text-} and \textit{image-} data. \citet{bodria-2021} provide a taxonomy where they match the input data type to explanation types. For text-data they identify \textit{sentence highlighting}, \textit{attention-based techniques} and rxplanations by example (prototypes and counterfactuals) as relevant. In terms of the explanation types introduced in \ref{explanationType}, sentence highlighting and attention based techniques can both be considered to produce feature importance scores (see \ref{methodType}). \citet{bodria-2021} further assign feature importance methods and rule extraction techniques to tabular-data. Saliency maps and concept attribution are assigned to image-data. While the mapping of input data type and explanation type provides a taxonomy that is easy to navigate, it has some exceptions. For example Anchor can also produce rules for textual input data \citep{ribeiro-2018,bodria-2021}.

\subsubsection{Dimension: Method Type}
\label{methodType}
Another common approach to distinguish explainability techniques is based on the similarities of techniques, which leads to the formulation of method types.
For model agnostic explanations, the following categories are defined throughout the survey papers:
\begin{itemize}
    \item \textbf{Erasure/Perturbation based methods}: Perturbation or erasure based methods inspect how the output of a model changes, by randomly or orderly switching, removing or replacing parts of an input for which the original output should be explained \citep{covert-2020,danilevsky-2020}.
    \item \textbf{Prototype selection methods}\PL{Is this a method type or an explanation type? --> CL: I think it would be closely related to explanation by example approaches. I.e. a family of methods that returns this kind of output type} return additional input samples for which a model would return a similar score as for given sample \citep{guidotti-2018}. \citet{guidotti-2018} consider this approach in the context of building an interpretable model, by using prototypes as a base for further decisions. 
\end{itemize}
In contrast, the following categories are exemplary for methods specific to neural networks:
\begin{itemize}
    \item \textbf{Activation Maximization methods} check, which inputs maximize the output(s) (e.g. for single neurons or the overall prediction) \citep{guidotti-2018, montavon-2018}.
    \item \textbf{Attention-based methods:} The widely used transformers architecture by \citet{vaswani-2017} is based on attention layers that learn which part in an input to attend to, i.e. which parts of an input are most important to pass to the next layers. As attention has the intuition of showing, which parts of the input a model has learned to treat as important, some works apply attention as a technique to provide further understanding of the model's decision process \citep{danilevsky-2020, bodria-2021}. However, there is an ongoing debate about the usefulness of this approach (mostly regarding RNN architectures). E.g. \citet{jain-2019} show that attention methods are often only weakly correlated with other approaches that assign importance scores to input features. \citet{wiegreffe-2019} note the broad range of definitions for explainability, thereby allowing attention scores to be treated as explanations, even when they do not fully represent a model's "internal workings", as they could still be plausible to human users. \citet{bastings-2020} also argue that gradient based, propagation based and erasure based methods are preferable over attention to explain a model's decision to a model developer. They work out that attention based methods are only reflecting a model's state at a certain point whereas the other approaches take the whole model into account. 
    \item \textbf{Gradient-based methods} :
    Gradient-based methods are usually used to compute feature importance scores by evaluating the gradients with respect to the input features of the original or permuted inputs \citep{danilevsky-2020}. This is especially useful for neural networks, as gradients can be computed via backpropagation.
    \item \textbf{Layerwise relevance propagation (LRP)}: Layer wise relevance propagation techniques, first coined in \citet{bach-2015}, assign predefined rules to each type of layer (e.g. fully connected, convolutional, ...) that have the goal to decompose the output onto the inputs by going backwards through the network \citep{montavon-2018, danilevsky-2020}.
\end{itemize}
Most of the techniques in these categories return feature-importance scores. There is a number of distinctions that we don't cover here, such as Sensitivity Analysis \citep{guidotti-2018}, that \citet{danilevsky-2020} consider to be an old concept similar to gradient based approaches. The method types can overlap. For example, techniques for LRP or input perturbations might also leverage gradients.

%\subsubsection{Dimension: User Experience}
%\citet{doshi-velez-2017, guidotti-2018} propose the dimension of user experience to differentiate techniques based on their target audience. E.g. in MT evaluation a single score for a translation, i.e. the usual output of a metric, might be sufficient for an expert to make a decision on its quality. For a non-expert however, it might not be enough and explanations with more details is more desirable.

%\subsubsection{Dimension: Time}
%\citet{doshi-velez-2017, guidotti-2018} further propose the dimension of the time that is required for a human user to understand an explanation. However \citet{guidotti-2018} note that there are not many works that actually test this dimension.

==> legacy/old_introduction.tex <==


The field of natural language generation (NLG) has undergone rapid progress in recent years \citep{gatt-2018}. NLG comprises subtasks such as Summarization, Image Captioning, Machine Translation (MT), dialogue, and many others  \citep{celikyilmaz-2020}. %Here, we set our focus on MT.
Our focus in this work is on MT. 
%NLG considers the automatic construction of human understandable text \citep{reiter-2000}.
%The goal of Summarization is to generate short summaries of longer texts \citep{shi-2021}. Image captioning considers the generation of natural language descriptions of images \citep{li-2019}. Finally, MT systems translate texts from a source language into a target language \citep{stahlberg-2019, yang-2020}. 
\PL{I think we can even start from MT without introducing NLG.}
MT is one of the most classical and challenging problems in Natural Language Processing, as it requires a deep understanding of meaning in order to produce a translation of a text in another language. %, as it requires that %translation systems capture the concepts of natural language \citep{reiter-2000}, a complex human concept. 
However, %the generation of translations is not the only difficulty of this domain. 
this is not the only problem. 
%Once systems are able to create reasonable outputs, it becomes desirable to assess their quality and to compare them. 
Evaluation of machine generated translations is %not only 
similarly 
essential for progress in the field, but also very challenging, as it requires to understand to which degree two sentences express the same meaning.\footnote{Can we argue that this is a difficult problem, but easier than generation?}  
%This evaluation requires an understanding of natural language, too. It needs to judge whether the translation is a good fit or not. Naturally, 
One option for evaluation of output quality %can be judged by human experts. 
involves humans. 
However, this is time consuming, expensive and infeasible to conduct at a large scale \citep{celikyilmaz-2020}. 
%Due to this reason, researchers have developed evaluation metrics to automatically check the quality of translations. 
Therefore, research has come up with a plethora of [...]
Thereby, it is desirable that the metrics correlate well with pre-collected annotations of the experts. 
MT metrics (and NLG metrics in general) compute the following operation:
$$\text{METRIC}(\text{HYP}, \text{GT}) = \text{SCORE}$$\todo{SE: I would not introduce a formula here}
The hypothesis (HYP) is the generated text that should be graded. The ground truth (GT) is additional information used to quantify the quality of the hypothesis. Often, it is comprised of one or multiple reference texts (REF), which are translated by human experts (reference-based metrics). Some metrics use the original source text (SRC)
of the HYP as GT.
% , which was translated into HYP. 
\PL{Maybe, we should introduce reference-based and reference-free metrics here.}

Early MT metrics are relatively easy to understand, as they follow a clearly defined algorithm and often could even be computed manually. For example, BLEU \citep{papineni-2002} computes a modified n-gram precision, i.e. 
% it checks 
checking
for the ratio of correctly predicted n-grams in the HYP to the overall number of predicted n-grams. METEOR \citep{lavie-2004,banerjee-2005} applies several rules to iteratively align words and then computes an F-measure based on unaligned words
to become the evaluation score.
BLEU and METEOR put a high emphasis on the precision. 
Meanwhile, metrics like ROUGE \citep{lin-2004}, which is often used in summarization, emphasize recall.
These three metrics compute lexical overlap, i.e. they check whether parts of the HYP are found in the REF (and/or vice-versa) without taking the actual meaning into account \citep{reiter-2018,zhao-2019}. Many prior works have shown that this is problematic \citep{ananthakrishnan-2006, reiter-2018}. Still, especially BLEU remains heavily used for evaluating MT systems to this date \citep{kocmi-2021}. 

Recently, a large number of soft MT metrics have been proposed to tackle the problems of lexical overlap metrics. ``Soft'' refers to the property that these metrics do not compare tokens directly, but rather compare their embeddings and thereby their meaning \citep{zhao-2020}. For example, \textit{BERTScore} \citep{zhang-2020} computes metric scores based on the maximum cosine similarities of contextualized word-embeddings \PL{of HYP and SRC ? --> in their paper of REF and HYP, but this is not relevant in this sentence, as it could also be used with SRC} extracted from BERT \citep{devlin-2019} (or other transformer language models). \textit{BLEURT} \citep{sellam-2020} is fine-tuned using an additional layer on top of a transformer model with human annotated scores. \textit{BARTScore} \citep{yuan-2021} leverages the generation probability a HYP has with BART \citep{lewis-2020} as metric score. In challenges for MT evaluation such as the WMT metrics shared tasks \citep{ma-2019,mathur-2020} and the WMT quality estimation shared tasks \citep{fonseca-2019, specia-2020}, transformer-based approaches \PL{Should we introduce briefly here what transformer is and mention that BERT/BART are also transformer-based? --> If we keep such a part, I'd cite the transformers paper but not say here what these are} have been shown to achieve state-of-the-art performance in terms of correlation with human judgments. %and the STSB challenge for semantic similarity \citep{cer-2017}

To summarize \PL{Hence, we can see that --> Not sure if "hence" is better here, as to me hence sounds like it is more refering to the last point}, there is a paradigm shift that improves metric quality, but at the same time introduces black-box language models into the process. While the ``decision process'' of BLEU and ROUGE was easy to understand, it is harder to explain the process of these newer soft MT metrics. \PL{hindering their --> not sure how to apply this here} Still, this understanding can be helpful for further improvement and acceptance, i.e. it becomes desirable to explain the metrics.

This paper connects the fields of explainable AI and MT evaluation. We build upon the specifics that set \textit{explainable MT evaluation} apart from other explainability tasks in NLP and design a conceptual framework. Further, we provide an overview of recent approaches and discuss, how each of them addresses these properties. We make the following contributions:
\begin{itemize}
    \item Based on work from the domain of eXplainable Artificial Intelligence (XAI), we define core concepts and goals of explainable MT evaluation.
    \item To the best of our knowledge, we provide the first taxonomy of works that are related to the explainability of MT evaluation metrics.\PL{Can we drop a teaser here how the taxonomy look? 
     --> This could also be the teaser on the properties themselves (if we keep this section, I would add it)} While most of them were \MF{Are we saying the explainability methods we discussed have already been applied to the field of MT evaluation? I don't think they were, right? I would rephrase that, smth like: "although we discuss how to apply them to MT evaluation..." 
    --> Yes, techniques that were applied to the MT domain are: "feature importance", "Bartscore (to some extend)", "Global expl.", "perturbation checklists"} applied to the domain of machine translation evaluation, we fathom that they could be applied to other NLG tasks with little change. 
    \item We conduct supplementary experiments to the recent Eval4NLP shared task \citep{fomicheva-2021} and provide an initial design for example-based explainability of metrics. Our experiments show surprising results for word-level explanation capabilities of lexical overlap metrics and further call into question the usage of model-agnostic post-hoc explainability techniques to explain metric scores.\PL{This comes out of the blue. Shall we introduce it somehow earlier? --> I think we will handle this in the new intro section}
    \item We identify open research questions and suggest techniques to consider in future work.
\end{itemize}

We structure our work into ... sections. 

\todo[inline]{SE:
Why are explainable metrics special?
- formally: 
  (i) pairs of texts, not single text classification
  (ii) regression task, not classification
  ...
- other:

Why are explainable metrics important?
- user trust
- metric crisis (researchers still don't trust/user BERT-based metrics)
- new metrics may have limitations, which we need to unveil
- ...

CL: Should these points already be mentioned in the introduction? Currently they can be found in section 2, where goals and properties are described. 
}

==> legacy/old_structure/1.1_metrics.tex <==
\section{Evaluation Metrics (for Machine Translation)}

% Todo: remove other current section on this topic
%A main difficulty of Machine Translation is to evaluate the quality of the hypothesis. For most sentences it is possible to produce another sentence conveying the same meaning in an equally natural way. And if multiple sentences are produced, the meaning of a single sentence could be spread.

%Machine translations can be evaluated with machine translation evaluation (MTE) metrics. 
%To give an overview of the characteristics of %these 
%evaluation metrics (for MT), we summarize the main dimensions along which the techniques used in this area can be ordered and differentiated.
\subsection{Metric Dimensions}

We first differentiate evaluation metrics for machine translation along several dimensions. A summary is shown in Table \ref{table:metrics}.\footnote{We note that different categorizations of metrics are possible and we propose one that }

\begin{table}[!htb]
\centering
\begin{tabular}{c|cccc}
     \toprule
     \textbf{Dimension} &  \textbf{Description} & \textbf{Examples} \\ 
     \midrule
     \emph{Degree of automation} & \\ \hline
     \emph{Use of embeddings} & Whether metrics take semantics into account\\ \hline 
     \emph{Supervision} & The degree of supervision a metric requires \\
     Training & \\
     Use of references & \\ \hline
     \emph{Metric task} & \\ 
     \bottomrule
\end{tabular}
\caption{}
\label{table:metrics}
\end{table}


%\iffalse
%\subsection
\paragraph{Degree of Automation}
This dimension describes the degree to which the evaluation of translations is automated or manual work \citep{celikyilmaz-2020}: %\\

\begin{itemize}
\item\textbf{Human Machine Translation Evaluation:} 
%\citet{van-der-lee-2019} describe that natural language is a human construct and therefore the correctness of a translation can be best graded by human experts. However, they also note that this 
Human evaluation is often still considered the gold-standard \citep{van-der-lee-2019},  %kind of evaluation 
but is expensive and slow. 
%Especially, when training a new system for MT, feedback for a generated translation must be given for each output, which quickly becomes infeasible when thousands of samples should be graded every minute. Therefore, human evaluation is mostly used to assess the quality of MT systems after training and as a base to construct and evaluate automated metrics. The other dimensions described below only apply to automated metrics.

\item\textbf{Automated Machine Translation Evaluation:}
%In contrast to human MTE, 
Automated MTE does not require manual input during runtime. Depending on the metric, they might however require one or more reference translations in order to judge a hypothesis. %(see reference-based vs. reference-free). 
Such metrics are typically fast enough to grade hypotheses during training or validation steps \citep{van-der-lee-2019}. However, they do not perfectly correlate with human judgments, which affects the translation quality reachable by MT systems.

\item\textbf{Semi-Automated Machine Translation Evaluation:}
It is also possible to combine manual human input with automated metrics. For example, \citet{hashimoto-2019} use human evaluation to capture quality, and statistics to capture diversity in the NLG domain. 
%This is done under the assumption that it is not easy to check for a human, whether a model is just using phrases it has already seen during training or if it generates text more freely.
\end{itemize}
%\fi 

\paragraph{Usage of Embeddings}
%Embeddings are vector representations of textual or symbolic inputs. 
%Methods that learn 
Embeddings have seen great success in encoding linguistic information as dense vector representations \citep{mikolov-2013,devlin-2019}. The following distinctions of embedding usage can be found %across metrics for MTE 
in 
\citet{sai-2020}:
\begin{itemize}
\item\textbf{No Embeddings:}
%Some metrics use no embeddings. For example, 
Metrics such as BLEU \citep{papineni-2002} or NIST \citep{doddington-2002} are based on exact word matches between n-grams of hypothesis and reference sentences. METEOR \citep{lavie-2004,banerjee-2005} goes a step further and employs 
%, for example, 
a.o.\ stemming %algorithms 
to account for non-exact word matches. Nonetheless, all of these metrics do not check whether the meaning of two sentences is preserved and have difficulties to deal with paraphrases and %as well as %usage of %synonymous words 
synonyms 
\citep{ananthakrishnan-2006, reiter-2018}. These problems lead to a lower correlation to human judgements in segment-level evaluations %, which can for example be seen in evaluations performed by 
\citep{stanojevic-2015, mathur-2020}. 

\item\textbf{Static Embeddings:} %\citet{wang-2020} provide a survey of word-embeddings. They summarize that 
Static embeddings are vector representations %that are assigned in a fixed way. I.e., 
such that the representation of a token will %stay 
be the same across contexts \citep{mikolov-2013,pennington-2014}. %A word such as ``bass'', which could be a sea bass or an instrument, would receive the same vector representation. Further, they summarized that embeddings like one-hot-encodings are used to present tokens as numbers, which enables mathematical operations. 
%Dimensionality-reduced embeddings additionally would allow to encode properties such as \textit{meaning} into the vector representations. 
%Thereby, textual units can be compared by %distance metrics. In one-hot encoding, all words have the same relation, e.g. a fish is as similar to a whale as to an elephant. 
%In dense representations such as Word2Vec \citep{mikolov-2013} or GloVe \citep{pennington-2014} a word like `fish' might lie closer to the whale. 
The use %introduction 
of static embeddings in MTE allows to compare sentences that use different words than a reference but express the same content \citep{fishel-2017}. Examples of metrics based on static word embeddings are %for metrics that use static word embeddings are 
bleu2vec \citep{fishel-2017} and XYZ.\todo{SE: Add a better second example.} 
%sentence mover's similarities \citep{clark-2019}  (they also use contextualized embeddings). 

\item\textbf{Contextualized Embeddings:}
Contextualized embeddings assign vector representations depending on an input context \citep{wang-2020,devlin-2019}. 
%Depending on the context surrounding a token, these representations can differ between words such as ``bass'', that can have a different meaning in different contexts. 
%Additionally, they allow to find words that are close to each other in a specific context. This type of embedding is usually achieved by leveraging the hidden states of a transformer model after a forward pass of the tokens that should be encoded. 
%In MTE, this allows to compare the meaning of sentences rather than whether their words have similar meanings in general. 
Comparison between sentences in MTE that build on contextualized representations can be on word-level \citep{zhang-2020, zhao-2019} or by comparing embeddings of the whole sentence \citep{reimers-2020}. The currently best-performing metrics build on contextualized representations \citep{}. 

\end{itemize}
As metrics without embeddings perform a strict comparison between words, we will refer to them as \textit{hard} metrics \citep{zhao-2020}. In contrast, metrics that use embeddings are referred to as \textit{soft} metrics.

%\subsubsection{Reference-Based vs. Reference-Free}
\paragraph{Supervision}
This dimension distinguishes whether an automated MTE metric %is using references or the source as a base of grading the hypothesis.\\
uses a form of supervision or not. 
\begin{itemize}
\item\textbf{Reference-Based:} We call a metric %is called 
reference-based if it requires one or multiple human reference translations to compare with the hypothesis, which can be seen as a form of supervision. %\citep{zhang-2020}. %Thus, this technique requires preceding human effort to generate ground truth translations and is more expensive. Additionally, this kind of 
% References can be seen as a form of supervision. 
 Such a metric cannot be used in cases where no bilingual expert %speaking both languages 
is available. 

\item\textbf{Reference-Free:} 
%In contrast, 
Reference-free metrics do not require a reference translation to grade the hypothesis \citep{zhao-2020,ranasinghe-2020}. 
Instead, they %are based on the similarity to the source to determine the quality. 
directly compare the source to the hypothesis. 
%When multilingual embeddings are trained, there is an intuition that words with similar context in different languages should be close to each other. 
%This is leveraged by using distance measures \citep{zhang-2020,zhao-2020} on these embeddings or by directly learning to predict human-like scores \citep{sellam-2020}. 
In the literature, reference-free MTE is also referred to as ``reference-less'' or (especially in the MT context) ``quality estimation''. 

%\item\textbf{Combining source and reference sentences:} The recent metric COMET \citep{rei-2020} combines the usage of source and reference sentences to achieve a better correlation with human judgements in predicting the score of the hypothesis.
\end{itemize}

%\subsection{Untrained vs. Trained}
Another distinction is whether a metric is untrained or trained, i.e.\ whether it has trainable weights that are fitted in order to solve the task of MTE \citep{celikyilmaz-2020}:
\begin{itemize}
\item\textbf{Not Trainable:} This dimension indicates that a metric has no learnable weights. %This is fitting for metrics such as BLEU or METEOR that do not use learned representations of words or sentences. 
\item\textbf{Pre-Trained:} Some metrics leverage embeddings that were trained in more general tasks without fitting them to the task of MTE. This is the case for BERTScore \citep{zhang-2020} and MoverScore \citep{zhao-2019} which extract contextualized embeddings from language models.

\item\textbf{Fine-Tuned:} Finally, some metrics directly optimize the correlation of metric scores with human judgment in a supervised learning setup. 
%Therefore, they often leverage the human labeled data from previous shared tasks on metric evaluation. 
Samples for this type of metric are BLEURT \citep{sellam-2020}, COMET \citep{rei-2020}, and TransQuest \citep{}. 
\end{itemize}

%\subsection
\paragraph{Metric Task}
\citet{yuan-2021} describe a further distinction based on the task a metric is designed to solve in order to achieve correlation with human judgment. They identify the following tasks:
\begin{itemize}
    \item \textbf{Unsupervised Matching:} They place all metrics that match hypothesis and reference tokens in this dimension. In terms of the dimension ``untrained vs. trained'' unsupervised matching captures metrics that are ``not-trainable'' or ``pre-trained''.
    \item \textbf{Supervised Regression:} These models use supervised regression to train a model to predict continuous values that directly correlate with human judgments from hypothesis and reference tokens.
    \item \textbf{Supervised Ranking:} In this setup, the model is trained to rank hypothesis sentences. For example, \citet{rei-2020} propose a regression and a ranking setup. In the ranking setup they minimize a loss that becomes smaller the greater the distance between embedding representations of the two sentences become.  
    \item \textbf{Text Generation:} 
    %In this setup 
    The authors place the metric PRISM \citep{thompson-2020} and their own metric BARTScore in this condition. BARTScore leverages the fact that a model that is trained to generate a hypothesis from a reference or source is at the same time trained to maximize the correlation to human judgement. They take variants of BART \citep{lewis-2020}, a model for text generation, that where finetuned on different tasks (summarization and paraphrasing). Then they use one of source, hypothesis or reference as input and one as ground truth for loss computation. This allows them to calculate the generation probability of the ground truth given the input. For translation evaluation they take the arithmetic mean of the directions reference $\rightarrow$ hypothesis and hypothesis $\rightarrow$ reference.
\end{itemize}
%It is to note 
%We note that \citet{yuan-2021} only feature the reference-based case in their description of the dimensions ``Unsupervised Matching'' and ``Supervised Regression''. With e.g. BERTScore \citep{zhang-2020} with multilingual embeddings \citep{song-2021} for ``Unsupervised Matching'' or MonoTransquest \citep{ranasinghe-2020} for ``Supervised Regression'' this dimension also applies to the reference-free dimension.


\subsection{Evaluating metrics}
%Machine translation 
Evaluation metrics %themselves 
can be evaluated by checking their correlation to human scores on manually labeled datasets. In the following we summarize procedures for collecting human scores: 
\begin{itemize}
    \item \textbf{Direct assessment (DA) of translation adequacy} This type of human scoring is proposed by \citet{graham-2015} and was applied in recent iterations of the WMT metrics shared task \citep{bojar-2017, ma-2018, ma-2019, mathur-2020} and the WMT quality estimation shared task \citep{fonseca-2019, specia-2020}. Annotators are presented with a hypothesis and reference sentence in reference-based setups or a source sentence in reference-free setups. They are then tasked to rate the similarity of their meaning on a (5-point) scale between 0 and 100. %The scores are z-scored for every annotator to align them with each other. 
    In the metrics shared task, the scores are used for \emph{system-level evaluation} by averaging them for each annotator per sentence for each system.\todo{SE: first one averages over annotators and then one assigns a system the average (averaged) score over all sentences, right?} Segment-level scores in the metrics shared task of WMT17 are collected in the same way but with a larger number of annotators to emphasize reproducibility \citep{bojar-2017}. They are averaged across annotators to produce segment-level scores.\todo{SE: need to describe how sys-level and seg-level evaluation is actually conducted} To be able to use a lower number of annotations per sentence, in the WMT18 to WMT20 metrics task, the segment level scores were reformulated into a ranked comparison based on DA scores \citep{ma-2018, ma-2019, mathur-2020}. If the average DA scores for two translations are over 25\% apart, they are considered in the ranking.\todo{SE: What is the purpose?} Since WMT19 the quality estimation shared task considers direct assessments for segment level evaluation, too \citep{fonseca-2019}. The DA annotation scheme of the WMT20 quality estimation \citep{specia-2020} shared task is using a ten-point scale instead of a five point scale following the setup by \citet{guzman-2019}.
    \item \textbf{HTER:} HTER (Human-Targeted Translation Edit Rate) is an evaluation method by \citet{snover-2006}. Human annotators are tasked to correct hypothesis sentences with as little edits as possible. The HTER is the number of edits that was necessary. This metric is for example used in the WMT tasks for quality estimation \citep{fonseca-2019, specia-2020} and in the MLQE \citep{fomicheva-2020b} and MLQE-PE \citep{fomicheva-2020} corpora that partly overlap with the datasets used in these shared tasks.\todo{SE: which shared tasks?}  Other than DA, the HTER is negatively correlated with similarity scores. As the method counts the edits in a sentence, it can be easily applied on a word level to flag which words are erroneous and which ones are ok \citep{fonseca-2019, specia-2020}.
    \item \textbf{MQM:} \label{MQM} MQM (Multidimensional Quality Metrics) is an annotation method in which multilingual annotators assign fine grained error labels to translations \citep{lommel-2014, lommel-2015}. In a recent evaluation, \citet{freitag-2021} compare %the usage of 
    DA and MQM. They label English-German and Chinese-English datasets with an MQM annotation scheme. The scheme uses main categories such as accuracy, fluency, style and terminology as well as several subcategories. Errors can be major, minor or neutral. A sentence score is inferred by computing the sum of differently weighted errors (and averaging them). The authors find that DA scores do not correlate well with MQM scores. Additionally, they find that MQM scores can distinguish human translations better from machine translations than DA scores (by ranking translations based on the scores). This calls into question the usability of DA-scores. They further show that the ranking of MT Systems and MTE Metrics can change based on whether DA or MQM scores are used. For this reason they switch to MQM based evaluations for the evaluations in the WMT21 metrics shared task \citep{freitag-2021b}.
\end{itemize}

Evaluations can be conducted on a system-, segment- and word-level \citep{specia-2020,mathur-2020}. Word-level evaluations have been conducted for the WMT task for quality estimation \citep{specia-2020}. The goal is to assign a label to each word and gap between them that indicates whether\todo{SE: what?} is erroneous or not. The Eval4NLP shared task \citep{fomicheva-2021} interprets word-level scores as explanations, when they are used in the computation of a sentence-level score. Segment-level evaluation compares scores that are assigned on the level of one or multiple sentences and system-level evaluation compares estimates on how good translation systems are performing \citep{mathur-2020}.\todo{SE: system-level evaluation compares metric scores on system-level to human scores on system-level?} Another option is evaluation on a document-level \citep{mathur-2020}.\todo{SE: system- and segment-level have been introduced before, maybe reduce redundancy}

Typical measures of correlation to human scores (for system- and segment-level evaluation) are Pearson- and Kendall- (for ranking based comparisons) correlation coefficients \citep{sai-2020}. 


==> legacy/old_structure/1_introduction.tex <==
\todo[inline]{SE: link to abstract: \url{https://docs.google.com/document/d/1AjVKc1-bkbnf9YJJKz0lKuLz1LAW_SYemAqfZyWly8M/edit}}

\todo[inline]{SE: I would suggest a structure such as: 1. Introduction; 2. Evaluation Metrics; 3. Explainability (shorter than currently); 4. Explainability for Metrics; 5. Taxonomy of current approaches and approaches themselves; 6. Our extensions (especially adversarial approaches); 7. Prospective future approaches; 8. Discussion, Conclusion, etc.}

\section{Introduction}
%\todo[inline]{SE: alternative introduction: 
{
The field of evaluation metrics for Natural Language Generation (NLG) is currently in a deep crisis: %While novel approaches to evaluation have been introduced in the last several years (and continue to get invented) that show relatively high correlation with human assessments of text generation quality \citep{}, 
While multiple high-quality evaluation metrics \citep{zhao-2019,zhang-2020,rei-2020,sellam-2020,yuan-2021}
%\todo{SE: add others} 
have been developed in the last few years, 
the Natural Language Processing (NLP) community seems reluctant to adopt %these novel high-quality metrics 
them to assess NLG systems. %Instead, 
In fact, the empirical investigation of \citet{marie-etal-2021-scientific} shows that the vast majority of machine translation (MT) papers 
%the community mostly still 
(exclusively) relies on surface-level evaluation metrics like BLEU and ROUGE \citep{papineni-2002,lin-2004} for evaluation, which were invented two decades ago, and the situation has allegedly even worsened recently.  
%but which are fundamentally flawed, and consequently typically have poor correlations with human assessments \citep{}. 
These surface-level metrics cannot measure semantic similarity of their inputs and are thus fundamentally flawed, particularly when it comes to assessing the quality of recent state-of-the-art NLG systems \citep{peyrard-2019-studying}, calling the credibility of a whole scientific field in question.\todo{SE: that's the title of Marie et al.}
%[Now we can speculate about the reasons (e.g., comparing to previous results is probably a main reason), but we can especially emphasize the black-box nature of the metrics and the ensuing explainability need, which is the main goal of our work]

Among the potential reasons for this %state-of-affairs 
neglect of recent high quality metrics 
are: (i) non-enforcement by reviewers; (ii) easier comparison to previous research, e.g., by copying results from tables of related work  (potentially a pitfall in itself); (iii) [others?]; (iv) lack of trust in and transparency of high-quality black box metrics.

In this work, we concern ourselves with the last named reason, explainability. [now say something why explainability is crucial and critical in AI and then for Evaluation Metrics]\todo{SE: explainability helps post-editing, btw.}

[then say something about our contributions:]
First, we provide a summarizing and synthesizing  overview\todo{SE: along with a taxonomy and classification?} over the first works from the novel research field of Explainable Evaluation Metrics. 
%which has emerged in 2021. 
Among those are [...]. Then we extend this line of research by focusing on the relationship between explainability and adversarial attacks \citep{}, which\todo{SE: why is this missing? why is this crucial?}. Finally, we provide requirements and schemata for potential future explainable evaluation metrics\todo{SE: why isn't the research not yet finished and why will this continue to be important in the future?} 
[The quest for explainable metrics is likely to continue (by no means have we seen its end already), thus we provide ...]

Our work is structured as follows. 
}
%With the recent advancements of neural networks, 

\todo[inline]{SE: original intro  below}


The field of natural language generation (NLG) has undergone rapid progress in recent years \citep{gatt-2018}. NLG comprises subtasks such as Summarization, Image Captioning, Machine Translation (MT), dialogue, and many others  \citep{celikyilmaz-2020}. %Here, we set our focus on MT.
Our focus in this work is on MT. 
%NLG considers the automatic construction of human understandable text \citep{reiter-2000}.
%The goal of Summarization is to generate short summaries of longer texts \citep{shi-2021}. Image captioning considers the generation of natural language descriptions of images \citep{li-2019}. Finally, MT systems translate texts from a source language into a target language \citep{stahlberg-2019, yang-2020}. 
\PL{I think we can even start from MT without introducing NLG.}
MT is one of the most classical and challenging problems in Natural Language Processing, as it requires a deep understanding of meaning in order to produce a translation of a text in another language. %, as it requires that %translation systems capture the concepts of natural language \citep{reiter-2000}, a complex human concept. 
However, %the generation of translations is not the only difficulty of this domain. 
this is not the only problem. 
%Once systems are able to create reasonable outputs, it becomes desirable to assess their quality and to compare them. 
Evaluation of machine generated translations is %not only 
similarly 
essential for progress in the field, but also very challenging, as it requires to understand to which degree two sentences express the same meaning.\footnote{Can we argue that this is a difficult problem, but easier than generation?}  
%This evaluation requires an understanding of natural language, too. It needs to judge whether the translation is a good fit or not. Naturally, 
One option for evaluation of output quality %can be judged by human experts. 
involves humans. 
However, this is time consuming, expensive and infeasible to conduct at a large scale \citep{celikyilmaz-2020}. 
%Due to this reason, researchers have developed evaluation metrics to automatically check the quality of translations. 
Therefore, research has come up with a plethora of [...]
Thereby, it is desirable that the metrics correlate well with pre-collected annotations of the experts. 
MT metrics (and NLG metrics in general) compute the following operation:
$$\text{METRIC}(\text{HYP}, \text{GT}) = \text{SCORE}$$\todo{SE: I would not introduce a formula here}
The hypothesis (HYP) is the generated text that should be graded. The ground truth (GT) is the information based on which the HYP is graded. Often, it is comprised of one or multiple reference texts (REF), which are translated by human experts (reference-based metrics). Some metrics use the original source text (SRC)
of the HYP as GT.
% , which was translated into HYP. 
\PL{Maybe, we should introduce reference-based and reference-free metrics here.}

Early MT metrics are relatively easy to understand, as they follow a clearly defined algorithm and often could even be computed manually. For example, BLEU \citep{papineni-2002} computes a modified n-gram precision, i.e. 
% it checks 
checking
for the ratio of correctly predicted n-grams in the HYP to the overall number of predicted n-grams. METEOR \citep{lavie-2004,banerjee-2005} applies several rules to iteratively align words and then computes an F-measure based on unaligned words
to become the evaluation score.
BLEU and METEOR put a high emphasis on the precision. 
Meanwhile, metrics like ROUGE \citep{lin-2004}, which is often used in summarization, emphasize recall.
These three metrics compute lexical overlap, i.e. they check whether parts of the HYP reoccur in a REF (and/or vice-versa) without taking the actual meaning into account \citep{reiter-2018,zhao-2019}. Many prior works have shown that this is problematic \citep{ananthakrishnan-2006, reiter-2018}. Still, especially BLEU remains heavily used to this date \citep{kocmi-2021}. 

Recently, a large number of soft MT metrics have been proposed to tackle the problems of lexical overlap metrics. ``Soft'' refers to the property that these metrics do not compare tokens directly, but rather compare their embeddings and thereby their meaning \citep{zhao-2020}. For example, \textit{BERTScore} \citep{zhang-2020} computes metric scores based on the maximum cosine similarities of contextualized word-embeddings extracted from BERT \citep{devlin-2019} (or other transformer language models). \textit{BLEURT} \citep{sellam-2020} is fine-tuned using an additional layer on top of a transformer model with human annotated scores. \textit{BARTScore} \citep{yuan-2021} leverages the generation probability a HYP has with BART \citep{lewis-2020} as metric score. In challenges such as the WMT metrics shared tasks \citep{ma-2019,mathur-2020} and the WMT quality estimation shared tasks \citep{fonseca-2019, specia-2020}, transformer-based approaches \PL{Should we introduce briefly here what transformer is and mention that BERT/BART are also transformer-based?} have been shown to achieve state-of-the-art performance in terms of correlation with human judgments. %and the STSB challenge for semantic similarity \citep{cer-2017}

To summarize, there is a paradigm shift that improves metric quality, but at the same time introduces black-box language models into the process. While the ``decision process'' of BLEU and ROUGE was easy to understand, it is harder to highlight the process of these newer metrics. Still, this understanding can be helpful for further improvement and acceptance, i.e. it becomes desirable to explain the metrics.

This work \PL{You mean our paper or explaining MT metrics work in general?} connects the fields of explainable AI and MT evaluation. We build upon the specifics that set \textit{explainable MT} apart from other explainability tasks in NLP and design a conceptual framework. While we put our focus on MT evaluation, we note that most of the concepts can be applied to NLG evaluation metrics in general. \PL{This probably goes to the conclusion or later sections. Let us focus on MT first.} Further, we provide an overview of recent approaches and discuss, how each of them addresses these concepts. We make the following contributions:
\begin{itemize}
    \item Based on work from the domain of eXplainable Artificial Intelligence (XAI), we define core concepts and goals of explainable MT evaluation.
    \item To the best of our knowledge, we provide the first taxonomy of works that are related to the explainability of MT evaluation metrics.\PL{Can we drop a teaser here how the taxonomy look?} While most of them were applied to the domain of machine translation evaluation, we fathom that they could be applied to other NLG tasks with little change. 
    \item We conduct supplementary experiments to the recent Eval4NLP shared task \citep{fomicheva-2021} and provide an initial design for example-based explainability of metrics. Our experiments show surprising results for word-level explanation capabilities of lexical overlap metrics and further call into question the usage of model-agnostic post-hoc explainability techniques to explain metric scores.\PL{This comes out of the blue. Shall we introduce it somehow earlier?}
    \item We identify open research questions and propose techniques to consider in future work.
\end{itemize}

We structure our work into ... sections. 

\todo[inline]{SE:
Why are explainable metrics special?
- formally: 
  (i) pairs of texts, not single text classification
  (ii) regression task, not classification
  ...
- other:

Why are explainable metrics important?
- user trust
- metric crisis (researchers still don't trust/user BERT-based metrics)
- new metrics may have limitations, which we need to unveil
- ...

CL: Should these points already be mentioned in the introduction? Currently they can be found in section 2, where goals and properties are described. 
}

==> legacy/old_structure/2_terminology.tex <==
\section{Terminology and Goals}
\label{terminology}
In this section, we introduce the terminology we use throughout the paper and derive goals for explainable MT evaluation.\PL{Overall, should we mention approaches for XAI in general but not yet applicable or impossible in the context of MT evaluation?}

Prior work has noted that there is an ambiguous usage of the terms \textit{interpretability} and \textit{explainability} \citep{barredo-arrieta-2020, jacovi-2020}. Based on recent surveys, we identify the following distinctions: \PL{It is important to define interpretability and explainability, but the whole set of bullet points here may be too far away from MT.}
\begin{itemize}
    \item \textbf{No differentiation}: The term \textit{explainability} is relatively new, while \textit{interpretability} has been used for a longer time \citep{adadi-2018, abdul-2018, barredo-arrieta-2020}. Due to this reason, most earlier works use the term \textit{interpretability} \citep[e.g.][]{lipton-2016, ribeiro-2016, li-2017}. Some newer works explicitly state that they use the two terms interchangeably \citep{adadi-2018, carvalho-2019, miller-2019, jacovi-2020}. Other works that do not make a distinction are \citet{biran-2017, xu-2019, bhatt-2020, vassiliades-2021}. 
    
    \item \textbf{Explainability as umbrella concept}:  \citet{gunning-2017} present interpretable models as a subcategory of explainability. Likewise, \citet{doran-2017} define explainability as umbrella concept of \textit{comprehensibility} and \textit{interpretability}, where comprehensibility is the degree to which a model can generally be reasoned about by a human and interpretability describes that the mapping function between input and output can be understood in detail. 
    
    \item \textbf{Interpretability as precondition for explainabilty}: \citet{montavon-2018, gilpin-2019} describe interpretability as a precondition to explainability. The interpretability definition of \citet{gilpin-2019} equates interpretability with the concept of \textit{plausibility}\PL{I think it's more like \textit{understandability} rather than \textit{plausibility} in their work.}, which we describe later in this section. Further, they define \textit{completeness} as a further requirement for explainability, which equates the concept of \textit{faithfulness}\PL{Also, not sure if it is equivalent to faithfulness in their work.}. \citet{montavon-2018} take a different approach and describe interpretations as the mapping from an abstract domain (e.g. a neural network's weights) to an interpretable domain (e.g. words). Then, an explanation would highlight important details in the interpretable domain (e.g. which words are important).
    
    \item \textbf{Passive Interpretability, Active Explainability}: Some works use the two terms to distinguish the notion of whether a model's process, e.g. the algorithm or the role of parameters, can be passively understood, or whether explanations are actively generated that do not necessarily provide a direct insight. \citet{barredo-arrieta-2020} use this distinction and define interpretability as a synonym of transparency, i.e. how much introspection the model offers by passively looking at it. Based on an English dictionary entry, they define explainability as an active process ``to make something clear to understand'' that is targeted towards an audience. \citet{burkart-2021} note that a common definition would be that interpretability has the goal of understanding a model as a whole, while explainability describes the means of providing explanations on it, even if it is a black box. However, throughout their paper the terms are used interchangeably. \citet{bodria-2021} also define explainability as the capability to actively generate valid explanations for a model's behaviour, while interpretability is the capability of passively understanding a model's behavior. \citet{israelsen-2017} also use such a distinction. 
\end{itemize}

These viewpoints are illustrated in figure \ref{fig:InterprExpl}. In this survey, we follow the fourth viewpoint. I.e., we follow \citet{barredo-arrieta-2020} and view a model as explainable, if the model or some external instance (described as \textit{Explanator} in the figure) can actively provide explanations that make the decision process or the output more clear to a certain audience. On the other hand, we use the term \textit{interpretable}, if the model can be passively understood. These definitions are similar to the concepts of model transparency and post-hoc interpretability described by \citet{lipton-2016}. There is, however, an important difference in that the model itself can provide explanations, too. Lipton would count this type of explanations towards model transparency; however, it does not necessarily lead to interpretability as in the above definition. For example, in the Eval4NLP 2021 shared task \citep{fomicheva-2021}, word-level scores are used to explain sentence-level metrics (see section \ref{eval4nlp}). Thereby, the word-level scores can be extracted with post-hoc explainability techniques, e.g. with LIME \citep{ribeiro-2016} or Integrated Gradients \citep{sundararajan-2017} as \textit{Explanators}. On the other hand, a metric could inherently produce word-level scores together with sentence-level scores. Such metrics are explainable, as their more verbose output provides explanations for the sentence level. Still, they are not necessarily interpretable, as potentially underlying language models cannot be passively understood, e.g. by a human inspecting their parameters. In contrast, we consider metrics like BLEU as interpretable, as their full process can be understood by an audience with a reasonable background in computer science. 

\begin{figure}[!tbp]
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/IvE1.png}
    \caption{No Differentiation}
    \label{fig:InterprExpla}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/IvE2.png}
    \caption{Explainability as umbrella concept}
    \label{fig:InterprExplb}
  \end{subfigure}\\
  \begin{subfigure}[b]{0.49\textwidth}
  \centering
    \includegraphics[width=0.7\textwidth]{images/IvE3.png}
    \caption{Explainability as a step up from interpretability}
    \label{fig:InterprExplc}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/IvE4.png}
    \caption{Passive Interpretability, Active Explainability}
    \label{fig:InterprExpld}
  \end{subfigure}
  \caption{Viewpoints on Explainability and Interpretability}
  \label{fig:InterprExpl}
\end{figure}
\PL{Fig1D: Do arrow colors convey any meaning? Also, can we minimize the number of angles in the model-to-explanation arrow?}

%\citet{lipton-2016} highlights the difficulties in giving a concise definition of interpretability (here also explainability). One of the reasons he names is that there is a diverse set of goals followed throughout the literature. We summarize some of the key properties identified by other surveys:
\subsection{Goals of explainable MT evaluation}
Besides the different definitions of key terms being used throughout the literature, there are also differences in the goals sought to be fulfilled by explainability techniques \citep{lipton-2016,carvalho-2019,barredo-arrieta-2020}. 
%For explainable NLG, we work out the following goals:
%\begin{itemize}
%    \item \textbf{Accessibility} describes the goal of allowing non-experts to use a model by providing insights into it \citep{lipton-2016,barredo-arrieta-2020}.
%    \item \textbf{Confidence} is the goal of providing confidence estimations for a model's output to support further decision making \citep{lipton-2016,barredo-arrieta-2020}.
%    \item \textbf{Causality} describes the goal of using the information gained from a trained model to infer causal relationships \citep{lipton-2016,barredo-arrieta-2020}. This means, a model gives insights into real world correlations, which can then be used to design experiments that test for causality.
%    \item \textbf{Fair \& Ethical Decision Making} describes the goal of ensuring a model to be unbiased and to adhere to laws and regulations by understanding its decision process \citep{lipton-2016,barredo-arrieta-2020}. Explainability can improve fairness by supporting the selection of unbiased models.
%    \item \textbf{Informativeness} describes the goal of increasing the amount of information conveyed by or about a model \citep{lipton-2016,barredo-arrieta-2020}. For example, rather than providing only a probability for a predicted class, or a regression result, additional information such as "the model followed rule X" can provide further support. This can help in supporting decisions that are made based on a model's output. Additionally it can highlight the flaws of a model, so that it can be improved in further development efforts.
%    \item \textbf{Transferability} describes the goal of understanding a model's capability to generalize to unknown domains \citep{lipton-2016,barredo-arrieta-2020}. E.g. \citep{ribeiro-2016} describe an example where a model used the presence of snow to distinguish between wolfs and huskies. By using their technique \textit{LIME} this error became clear, leading to the understanding that the model would not generalize well.
%    \item \textbf{Trust}: \citep{lipton-2016,carvalho-2019,barredo-arrieta-2020} identify trust as an often pursued goal across several research papers. \citep{lipton-2016} states however that trust is a property that is difficult to define. They consider that trust in that a model makes the right decisions might be achieved by having a high accuracy but it might also be achieved by only having a high accuracy in the same situation as a human does. It might also be trusted if it operates well without being biased, e.g. treating some individuals differently to others based on race or gender. Likewise, some individuals might only trust a system following their own biases. Thus, most of the other goals on this list may or may not achieve the subjective property of trust. 
%    \item \textbf{Safety}: \citet{doshi-velez-2017} discuss that end-to-end systems are difficult to fully test. Therefore explanations can provide a measure of a systems safety. 
%    \\For this goal to be fulfilled it is important for the explanations to be \textit{faithful}, as discussed later in this section.
%\end{itemize}
%Besides these, sometimes other goals such as Privacy Awareness (does a model use sensitive information?) and Interactivity (does a model interact with a human?) are considered \citep{barredo-arrieta-2020}. 

Following the goal definitions of different surveys, we consolidate three main goals for explainable MT:
\begin{itemize}
    \item \textbf{Checking for social biases}: Learned metrics might be biased towards certain types of texts used during training. Biases could be detected by observing explanations where e.g. gender, political or racial aspects are flagged to be important  \citep{lipton-2016}. For example, explanations could show that a metric considers male names as more important than female names in the same scenario. Mitigating such biases involves goals such as Fair \& Ethical Decision Making, Informativeness and Trust \citep[e.g.][]{lipton-2016, barredo-arrieta-2020}. 
    
    \citet{freitag-2020c} show that metrics can also include biases towards reference sentences, i.e. a preference towards REF, even though there are other correct generation options. They also state that references would often include \textit{Translationese}, i.e. source artifacts that originate when human translators don't find a natural translation. As these are no social biases, we count explainability techniques that help with their detection towards the next goal.\PL{Shouldn't this paragraph go to the next bullet point then?}
    \item \textbf{Diagnose and improve metrics}: By explaining why a metric predicted a certain score for a machine translation, where humans would assign a different score, the weaknesses of an existing metric might be understood. This might enable architectural changes or the selection of different datasets leading to model improvement. Likewise, explaining the whole model can unveil if the metric follows desired general properties (see section \ref{globalExpPaper}) This encapsulates goals such as Informativeness and Transferability \citep[e.g.][]{lipton-2016, barredo-arrieta-2020}. 
    \item \textbf{Make metrics more expressive and accessible}: A metric that assigns a score on a sentence level is difficult to understand for non-experts, e.g. non-native speakers. If a metric provides further information such as which words it considers incorrect, it may become more accessible. Similarly, for an expert it might save time and discussions to be presented with such explanations. This use case involves the goals of Informativeness and Accessibility \citep[e.g.][]{lipton-2016, barredo-arrieta-2020}. Further, we hypothesize that accessibility plays an important role in metric selection and might be one of the reasons for the broad usage of BLEU. I.e. researchers might have build trust in BLEU, due to its long and wide usage. Hence, when explanations help to build trust into black-box metrics, the paradigm shift to newer metrics might be propelled.
\end{itemize}

\subsection{Properties of explainable MT evaluation\PL{If possible, I would call them \textit{Challenges for} explainable MT evaluation.}} \todo[inline]{MF: This bullet point list should say what makes explaining MT metrics different from explaining other NLP tasks. We need to provide a summarized version of this in the introduction. Some of the points are missing. Also, I would put them in a different order: 1) Multiple inputs. This bit is very important but I think a bit problematic in its current version. It assumes that source and translation play the same role in defining the quality. Also, we miss a very important fact: translation quality is a property that emerges from the relation between the original and translated words. One of the challenges is precisely to capture this when explaining the metrics. 2) Relation to translation errors (this is not necessarily a challenge, but an important property) 3) Importance of context. In other NLP tasks such as text classification, if we e.g. remove the words relevant to the topic, this usually flips the score, and is a simple indication that those words are relevant. Such simple approaches do not work for explaining MT evaluation. 4) Multilingual input (in the case of reference-free metrics) 5) Output scores 6) Varying scales} Next, we consider important properties of MT metrics that have an impact on explainability techniques: 
\begin{itemize}
    \item \textbf{Output Scores}: Most MT evaluation metrics return numeric output scores, however most explainability techniques are originally intended to be used with classification \citep{lertvittayakumjorn-2021}\PL{Not sure if you can cite my paper to support this claim.}. While some of them can be adapted easily (e.g. LIME), others require the definition of intervals for which certain conditions should be met (e.g. Anchor).
    \item \textbf{Varying Scales}: As many metrics are based on learned models, the outputs often are not fixed to a range between 0 and 1. Therefore, they cannot be directly interpreted as probabilities. This problem can be tackled by using an approach detailed in \citet{zhang-2020}. Here, the authors determine a lower boundary of the metric by averaging the scores of a large collection of dissimilar sentences. Then, they rescale all further computations of the metric with this baseline. However, while this leads to the score to be between 0 and 1 most of the times, it doesn't guarantee for it. 
    
    Another option is to normalize the scores to have a mean of 0 and a standard deviation of 1 (z-score).\PL{Is there any paper using this option. If there is, please cite it.} For a given dataset this guarantees that scores are centred around 0 and spaced comparably across metrics. However, the normalized scores of new or perturbed sentences might follow a different distribution and fall out of this range. Additionally, the outputs of the metrics could be skewed differently. E.g. for two metrics that return outputs between 0 and 1, one could be more pessimistic and usually assign lower scores than the other. This makes comparison difficult as e.g. a score of 0.7 can have a different meaning for 2 metrics.
    \item \textbf{Multiple Inputs}: The metrics take multiple inputs. Therefore, there are multiple options when local (see \ref{sec:dimensions}) explainability techniques are applied: \todo{YG: having a figure to illustrate/compare the options would be great.}
    \begin{itemize}
        \item \textbf{Explaining with respect to the Hypothesis}: Usually when Machine Translation is evaluated, the reference and/or source sentences are already given, for example, by a human annotator. Then, the metric can be used to generate a score that answers the question ``Is the hypothesis good with respect to the given source or reference?''. Explaining with respect to the hypothesis would additionally (try to) answer the questions ``Why did the metric assign a certain score for this hypothesis with respect to the given source or reference?'' and ``How do changes to the hypothesis affect the score?''. As the source and/or reference are considered as given when a Machine Translation is evaluated, we consider this setup to be the most important one. It can help to understand the shortcoming of the translation system, thereby enhancing the benefits of the metrics.
        \item \textbf{Explaining with respect to Source/Reference}: This would answer the additional questions of ``Why did the metric assign a certain score for this source or reference with respect to a given hypothesis?'' and ``How can we change the reference/source to affect the score in certain ways?''. We consider these explanations to be less important\PL{I would not say that it is less important, but it complements the results of the previous case, showing where in the SRC that the HYP performs well or poorly.}, as the source and reference are usually considered the ground truth of an evaluation. Therefore, it is not necessary to change them, as long as the integrity of the data is not questioned. They can however be interesting for model diagnosis to see whether the model considers the expected parts of a source/reference when grading the hypothesis.
        \item \textbf{Explaining with respect to all inputs}: The question of whether all inputs can be explained together largely depends on the choice of the explainability method. For example,  for Input Marginalization \citep{kim-2020}, the result will be the same as when the Hypothesis and Source/Reference are explained solely.\PL{Any reasons why?} However, for additive feature explanation methods such as SHAP \citep{lundberg-2017}, the goal is to find a contribution of each feature to the final score. Therefore, when a SRC/REF and HYP are explained together by this technique, the scores assigned to each of their tokens will contribute to the final score together. This is not desirable as it can lead to corresponding tokens between HYP and SRC/REF to be assigned with contradicting feature importances (one will be positive while the other is negative).\PL{Can they be both positives but with smaller values?} Additionally, doing this would invert the baseline of the attributions. As an example, assume we want to explain the reference-based metric score of a reference and a hypothesis. When we explain only the hypothesis, as described in the first bullet point, a baseline contribution could be determined by removing all words from the hypothesis (depending on the technique). Hence, the metric score is probably low, as it compares an empty sentence to a non-empty sentence. However, when the feature importance of reference and hypothesis is determined together, the baseline would be determined by comparing an empty hypothesis to an empty reference, leading to a high baseline score. 
    \end{itemize}
    As long as the technique is not specifically tailored to explain inputs of sentence pairs, we advise to run one evaluation with respect to the hypothesis and one evaluation with respect to the source/reference separately.\PL{And then combine the scores?} \PL{Should we give any advice here or later? It seems we are mixing survey of existing works with suggestions.} 
\end{itemize}
\subsection{Dimensions of Explainability}
\label{sec:dimensions}
Now that we have noted desiderata and properties of explainable MT, we describe dimensions that are used across the literature to describe the properties of explainability techniques. We leverage these dimensions to provide a taxonomy of recent approaches for explainable MT.

\subsubsection{Dimension: Explanation Type}
\label{explanationType}
Based on the previous definitions of interpretability and explainabilty an explanation is additional information that is provided by a model or a separate component in order to make the model's outputs more clear \todo{YG: more clear or clearer? } to a specific target audience. We highlight different types of explanations and discuss their application for MT evaluation:
\begin{itemize}
    \item \textbf{Text Explanations} are explanations in the form of generated texts providing information on a model's output \citep{lipton-2016}. For MT evaluation, such an explanation could be a text such as
    ``The hypothesis received a score of 0.8 as it captures all the facts of the reference, but has grammatical errors for word A and word B''.
    \item \textbf{Visualizations} are explanations in the form of plots, generated images and other, mostly non-symbolic representations \citep{lipton-2016,adadi-2018}. For MT evaluation, such an explanation could be a plot of dimensionality reduced word embeddings of a hypothesis and a reference, showing the distance in alignment between the two. This would for example help to explain XMoverScore and BERTScore, which are based on the distances of contextual word-embeddings.
    \item \textbf{Explanations by Example} present similar cases (as the current input/output pair) from a database of understood cases \citep{lipton-2016,adadi-2018}. In MT evaluation a score might be explained by presenting examples of hypothesis-reference or hypothesis-source pairs that achieved a similar score (by the same model). However, this leaves the deduction of actual similarities to the user or another model. Explanations by example can be further differentiated into \textit{prototypes, criticism and counterfactuals} \citep{ruping-2006, wachter-2018,adadi-2018, burkart-2021}. Prototypes are similar examples representing one or multiple input-output pairs. They are helpful if the presented example is well-analyzed. If prototypes are pre-computed, criticisms (discriminating samples) are instances that are not represented well by them, i.e. for which no good prototype can be found. Counterfactual explanations describe examples with minimal changes to the input that change the output in a noticeable way (in the case of classification changes the class).
    \item \textbf{Explanation by Simplification} is achieved by training a simpler model to mimic the results of a complex one \citep{barredo-arrieta-2020}. In MT evaluation this would for example be given if it would be possible to represent a BERT model as a decision tree that would then be considered an explanation.
    \item \textbf{Feature Importance/Relevance Explanations}\footnote{\citet{barredo-arrieta-2020} note that these terms are used interchangeably} are explanations that assign a relevance score for every input feature \citep{barredo-arrieta-2020}. For example, given a hypothesis "this is not a cat" and a reference "this is a cat" an explanation of a perfect MT metric should assign a high negative relevance to the word "not". 
    \item \textbf{Rule Based Explanations} consist of one or more decision rules that allow to predict the behavior of a model if the conditions of the rule are met \citep{adadi-2018}. This is especially useful for classification as it allows to simulate a model's outcome. In the case of MT metrics that return numeric outputs, the scale could be discretized and a rule could for example be ``if phrase A, B and C are present in a hypothesis, the score will be X''. %\citet{danilevsky-2020} refer to rule based approaches as \textit{declarative induction}.
    \item \textbf{Local Explanations:} There is a difference between the scope of local explainability methods and explainability methods that provide local explanations. While local explainability methods (see \ref{localMethods}) explain a model's output for a single input-output pair, a local explanation applies to the neighbourhood around the input \citep{lipton-2016}. \todo{YG: an example will help here. what it means by 'neighbourhood around the input'? a sentence similar to the hyp/ref/input sentence? }
    \item \textbf{Concept Attributions} describe, to what extent a user provided concept is fulfilled in the data \citep{bodria-2021}. \citet{bodria-2021} state that this type of explanation is used in some approaches in the area of computer vision. In MT evaluation, a user could for example provide categories for \textit{missing facts} or \textit{incorrect sentence structure}.
\end{itemize}
The different explanation types are not fully distinct \todo{orthogonal?}. E.g. \citet{ribeiro-2016} build simplified, linear models, whose weights can be used as local explanations for changes applied to specific input features.\PL{I would see simplification (using surrogate models) as a method.} Therefore, they provide local feature importance explanations by simplification.
\citet{lipton-2016, barredo-arrieta-2020} list the presented explanation types as post-hoc explanations only. Following the definition of explainability given above, in this work, we will also use these explanation types for those that are actively generated by the model itself. 

\subsubsection{Dimension: Local vs Global Explainablity}
\label{localMethods}
Another common distinction used in taxonomies is the one of local vs global explainability techniques \citep[e.g.][]{doshi-velez-2017,arya-2019,carvalho-2019, danilevsky-2020,bodria-2021}. Global techniques try to characterize the behaviour of a model as a whole. In explainable MT, global explanations give insight into the general factors a metric considers when assigning a score.
\todo{YG: it's a bit hard to imagine what a global explanation would be like for MT evaluation. We may need more explanations or discussions here.}
Local techniques in contrast, provide explanations of a single input-output combination. For example, given a reference translation "My dog is lovely" and a machine translation "My dog is angry" with a predicted score of 0.7, a local explanation describes why the metric predicted this score for this instance.\\
%\citet{guidotti-2018} further divide this distinction into outcome explanation, model inspection and model explanation. Outcome explanation thereby is synonymous to local explanations. Model explanation techniques are analogous to global techniques and model inspection techniques follow the goal of identifying a model's internal properties without necessarily providing global understanding. As an example \citet{guidotti-2018} refer to the forming of understanding of the role of certain neurons in a neural network through explanations. 

\subsubsection{Dimension: Model Agnostic vs Model Specific}
\label{agnost}
\citet{carvalho-2019, barredo-arrieta-2020, bodria-2021} differentiate between model-agnostic and model-specific techniques. Model-agnostic techniques can be applied to any type of model while model-specific techniques can only be applied to specific types of models. 

%\subsubsection{Dimension: Input Data Type}
%\citet{guidotti-2018,arya-2019,bodria-2021} distinguish explainability techniques based on the datatype the explained model takes as input. They differ between \textit{tabular-}, \textit{text-} and \textit{image-} data. \citet{bodria-2021} provide a taxonomy where they match the input data type to explanation types. For text-data they identify \textit{sentence highlighting}, \textit{attention-based techniques} and rxplanations by example (prototypes and counterfactuals) as relevant. In terms of the explanation types introduced in \ref{explanationType}, sentence highlighting and attention based techniques can both be considered to produce feature importance scores (see \ref{methodType}). \citet{bodria-2021} further assign feature importance methods and rule extraction techniques to tabular-data. Saliency maps and concept attribution are assigned to image-data. While the mapping of input data type and explanation type provides a taxonomy that is easy to navigate, it has some exceptions. For example Anchor can also produce rules for textual input data \citep{ribeiro-2018,bodria-2021}.

\subsubsection{Dimension: Method Type}
\label{methodType}
Another common approach to distinguish explainability techniques is based on the similarities of techniques, which leads to the formulation of method types.
For model agnostic explanations, the following categories are defined throughout the survey papers:
\begin{itemize}
    \item \textbf{Erasure/Perturbation based methods}: Perturbation or erasure based methods inspect how the output of a model changes, by randomly or orderly switching, removing or replacing parts of an input for which the original output should be explained \citep{covert-2020,danilevsky-2020}.
    \item \textbf{Prototype selection methods}\PL{Is this a method type or an explanation type?} return additional input samples for which a model would return a similar score as for given sample \citep{guidotti-2018}. \citet{guidotti-2018} consider this approach in the context of building an interpretable model, by using prototypes as a base for further decisions. 
\end{itemize}
In contrast, the following categories are exemplary for methods specific to neural networks:
\begin{itemize}
    \item \textbf{Activation Maximization methods} check, which inputs maximize the output(s) (e.g. for single neurons or the overall prediction) \citep{guidotti-2018, montavon-2018}.
    \item \textbf{Attention-based methods:} The widely used transformers architecture by \citet{vaswani-2017} is based on attention layers that learn which part in an input to attend to, i.e. which parts of an input are most important to pass to the next layers. As attention has the intuition of showing, which parts of the input a model has learned to treat as important, some works apply attention as a technique to provide further understanding of the model's decision process \citep{danilevsky-2020, bodria-2021}. However, there is an ongoing debate about the usefulness of this approach (mostly regarding RNN architectures). E.g. \citet{jain-2019} show that attention methods are often only weakly correlated with other approaches that assign importance scores to input features. \citet{wiegreffe-2019} note the broad range of definitions for explainability, thereby allowing attention scores to be treated as explanations, even when they do not fully represent a model's "internal workings", as they could still be plausible to human users. \citet{bastings-2020} also argue that gradient based, propagation based and erasure based methods are preferable over attention to explain a model's decision to a model developer. They work out that attention based methods are only reflecting a model's state at a certain point whereas the other approaches take the whole model into account. 
    \item \textbf{Gradient-based methods} :
    Gradient-based methods are usually used to compute feature importance scores by evaluating the gradients with respect to the input features of the original or permuted inputs \citep{danilevsky-2020}. This is especially useful for neural networks, as gradients can be computed via backpropagation.
    \item \textbf{Layerwise relevance propagation (LRP)}: Layer wise relevance propagation techniques, first coined in \citet{bach-2015}, assign predefined rules to each type of layer (e.g. fully connected, convolutional, ...) that have the goal to decompose the output onto the inputs by going backwards through the network \citep{montavon-2018, danilevsky-2020}.
\end{itemize}
Most of the techniques in these categories return feature-importance scores. There is a number of distinctions that we don't cover here, such as Sensitivity Analysis \citep{guidotti-2018}, that \citet{danilevsky-2020} consider to be an old concept similar to gradient based approaches. The method types can overlap. For example, techniques for LRP or input perturbations might also leverage gradients.

%\subsubsection{Dimension: User Experience}
%\citet{doshi-velez-2017, guidotti-2018} propose the dimension of user experience to differentiate techniques based on their target audience. E.g. in MT evaluation a single score for a translation, i.e. the usual output of a metric, might be sufficient for an expert to make a decision on its quality. For a non-expert however, it might not be enough and explanations with more details is more desirable.

%\subsubsection{Dimension: Time}
%\citet{doshi-velez-2017, guidotti-2018} further propose the dimension of the time that is required for a human user to understand an explanation. However \citet{guidotti-2018} note that there are not many works that actually test this dimension.

\subsection{Evaluation of Explainability}
Like explainability techniques themselves, their evaluation is challenging. As explanations can target different goals, evaluation setups might not fit across all tasks. A common requirement is that a technique fulfills the properties of \textit{Faithfulness} and \textit{Plausbility} \citep{jacovi-2020}. The first refers to the technique's capability of accurately explaining a model (in our case a metric). Plausibility on the other hand refers to the capability to give explanations that appeal to humans. It is important that both of them are fulfilled to some degree, which is emphasized by the example in figure \ref{fig:PlausibilityIssue}. An explainability technique that only fulfills plausibility does not necessarily add information about a metric, or why it returned a certain score. I.e. the technique could even provide results contradicting to the metric's output and be plausible. While these ``explanations'' might still have desired properties, they don't fulfill the definition of explainability and the explainabilty technique itself might be used as separate metric. An explainability technique that only fulfills faithfulness does not improve the understanding of the explained metric\PL{It helps us understand that the metric works irrationally though.}, as the explanation does not appeal to humans. For example, the metric \textit{word-level Transquest} \citep{ranasinghe-2021} could be seen as plausible explainability technique for the metric \textit{BLEURT} \citep{sellam-2020} (if the source is available). Likewise, BLEURT could be seen as a faithful explanation of itself \citep{ribeiro-2016}. Previous taxonomies suggest, that plausibility evaluation involves humans, while faithfulness evaluation applies metrics without human judgment \citep{deyoung-2020}. This is supported by \citep{jacovi-2020} who hypothesize that it is not possible to grade faithfulness when human judgments are involved. We highlight a number of evaluation approaches that were introduced to measure each of the properties.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{images/PlausibilityIssue.png}
    \caption{An example highlighting a shortcoming of plausibility. An explainability technique might generate plausible explanations, even when the model's output is incorrect.} \label{fig:PlausibilityIssue}
\end{figure}

\subsubsection{Plausibility}
\label{Plausibility}
Evaluation methods for plausibility need to consider, how well explanations can be understood by a human audience. Therefore, plausibility evaluation involves human judgments. 
\citet{Lertvittayakumjorn-2019} design multiple human evaluation experiments, two of which tackle plausibility:
\begin{itemize}
    \item \textbf{Justify an explanation:} They select samples for which a well-trained model has a high classification confidence. Then they explain outputs of the model with an explainability technique. By only presenting the most important features in the explanation, a human should predict the output of the model. 
    \item \textbf{Help humans decide in uncertain situations:} They select samples, for which a well-trained model has a low classification confidence. Then they explain them using an explainability technique. By presenting the most important and most negatively important features, as well as the model's output, a human should predict, whether a model is correct.
\end{itemize}
Due to the numeric output of MT evaluation metrics, these approaches are problematic, as other measurements of prediction confidence would need to be employed. Still, the evaluation of how explanations support human work \citep{doshi-velez-2017} is a paradigm that could be used for metrics with numeric output as well. For example, future work could consider to apply the notion of simulatabilty\PL{Is it really about plausibility?} \citep{lipton-2016} to evaluate the plausibility of metrics. Concretely, we could follow the approach by \citep{hase-2020}. In case of MT metrics, this approach would evaluate, how close participants of the evaluation can predict the score of a metric before and after receiving an additional explanation.

Rather than evaluating how explanations support humans in their task execution, other works evaluate the correlation to pre-annotated human explanations. \citet{fomicheva-2021b} follow this setting in machine translation evaluation and introduce a dataset with human-annotated rationales, which they use to compute the correlation with feature-importance explanations. Thereby, due to the alignment with human judgment, explainability techniques that generate explanations with a high correlation have a high plausibility (this dataset is described in more detail in section \ref{eval4nlpdata}).


\subsubsection{Faithfulness}
\label{Faithfulness}
As advocated by \citet{jacovi-2020}, most evaluation methods for faithfulness do not incorporate human judgments. The following are common techniques used throughout the literature:
\begin{itemize}
    \item \textbf{AOPC}: The area over the perturbation curve (AOPC) score is a metric introduced by \citet{samek-2017} in the domain of computer vision. It is computed as follows:
    $$AOPC=\frac{1}{L+1}(\sum_{k=0}^Lf(x_{MoRF}^{0})-f(x_{MoRF}^{k}))_p(x)$$
    $$x_{MoRF}^{0}=x$$
    $$\forall 1\leq k\leq L:\;x_{MoRF}^{k}=g(x_{MoRF}^{k-1},r_k)$$
    In relation to MT metrics, $f$ is the metric function. $x_{MoRF}^{k}$ is the original hypothesis with $k$ removed tokens. The tokens are removed in order of their feature-importance (MoRF means ``most relevant first''). The position of the next token is given by $r_k$ and the function $g$ handles the replacement or removal. The intuition behind this evaluation method is that the output probability $p(x)$ of a model should drop more if an important feature is removed than when an unimportant feature is removed. Hence, when the input features are removed one by one, based on their importance, the curve of predicted probabilities should first fall strongly and then flatten. Therefore, if the computed area over the curve of perturbation outputs is big, the feature-importance method is said to be faithful. In terms of MT metrics, the curve does not show the drop in predicted probabilities, but the drop in predicted metric scores.\PL{A figure of AOPC curve would be helpful.}
    
    A number of variations to this score have been proposed in the literature. \citet{deyoung-2020} don't remove the tokens one by one, but rather replace a certain percentage of most important features in each step (1\%, 5\%, 10\%, 20\%, 50\%). This might capture token dependencies between words, though there might for example also be dependant words of which one is removed in the 1\% step and one in the 5\% step. 
    
    Another variant is proposed by \citet{kim-2020}. $g$ is modified to replace with random likely words predicted by a language model, rather then removing or replacing with a fixed word. They propose this approach in order to prevent out-of-distribution problems when evaluating modified sentences.
    
    A very similar approach is called \textit{degradation tests} \citep{schulz-2020,chen-2021}. These additionally consider the least relevant perturbations and are based on the area between the curves.
     
    \item \textbf{Post-Hoc Accuracy} is a method for classification settings that measures how many of the original class predictions are still correct if only a set number of most relevant tokens is kept in the input \citep{chen-2018}. This could be adapted to metrics with numeric outputs by evaluating, how many of the metric predictions are still within a certain range after only the most relevant tokens are kept.
    
    \item \textbf{Glass-Box approaches}: Another option to measure the faithfulness of an explainability technique is to explain interpretable metrics or metrics that provide explanations themselves \citep[e.g.][]{ribeiro-2016,Decao-2020, fomicheva-2021,leiter-2021}. This provides a ``synthetic ground truth''. However, explaining interpretable metrics such as BLEU might be easier for the explainability techniques than to explain SOTA metrics like BLEURT. Most explainable metrics that provide explanations themselves are stronger than BLEU, but are not necessarily faithful.\PL{If they are not faithful, how can they be used to evaluate faithfulness of another explanation method then?} For example, consider a metric that generates an additional text description of a single metric score with respect to an input. If the text generation is learned based on human annotated explanations of human scores, there is no guarantee that the metric actually followed a certain process internally.
\end{itemize}    

Recent work has explored the out-of-distribution (ood) problem that comes with the fixed removal or replacement of inputs to explainability techniques and evaluation methods \citep{kim-2020, rychener-2020}. They consider that neural networks might not have learned how to react to inputs with unusual permuted features, leading to an insincere evaluation. We note that many of the above approaches are prone to this problem. \citet{kim-2020} use mask replacement to keep the perturbed sentences in-domain. However, we note that this introduces another black-box component into the evaluation metric of an explainability technique, which might be dangerous.

Another problem we see is that the explainability evaluation might be biased towards the explainability technique. E.g. if evaluation method and explainability technique both use word removal, they favour each other more than if one of them uses mask replacement. Likewise, an evaluation method that leverages mask replacement might favour explainability techniques that use language models. 
    
Due to these considerations, we see the evaluation of faithfulness as problematic.\todo{YG: you may say it needs more investigation; present it in a more positive tone :)}

%\subsection{Domain specific NLG metric Terminology}
%Some of the works discussed throughout this paper have been applied to subtasks of NLG. In this section. We define terminology that is specific to certain subtasks:
%\begin{itemize}
%    \item \textbf{Reference-Free vs Reference-Based:} These terms are usually used in the context of MT evaluation and could also be applied to other tasks of cross-lingual language generation. A metric is called reference-based, if it requires one or multiple human reference translations to compare with the hypothesis \citep{zhang-2020}. Thus, this technique requires preceding human effort to generate ground truth translations and is therefore more expensive. Additionally this kind of metrics cannot be used in cases where no expert speaking both languages is available. In contrast, \textit{reference-free} metrics do not require a reference translation to grade the hypothesis \citep{zhang-2020,ranasinghe-2020}. Instead, they use the similarity to the source sentence to determine the quality. In the literature, reference-free MT is also referred to as "reference-less" or "quality estimation". The recent MT metric Comet \citep{rei-2020} combines the usage of source and reference to achieve a better correlation with human judgments.

%\end{itemize}
%The surveys by \citet{sai-2020,celikyilmaz-2020} provide a good further overview.

==> legacy/old_structure/3_taxonomy.tex <==
\section{Taxonomy}
The next two chapters summarize recent approaches that are related to the concept of explainable MT evaluation. In table \ref{taxonomy}, we provide an overview of these methods in terms of the properties introduced throughout the section \ref{sec:dimensions}.\PL{At the moment, it is more like a survey than a critical analysis paper.} 

\begin{table*}[!htb]
\small 
\centering
\begin{tabular}{p{4.5cm}ccccccc}
     \toprule
     \textbf{Work} & \textbf{Type} & \textbf{L/G} & \textbf{A/S} & \textbf{Method} & \textbf{Eval} & \textbf{Goals} & \textbf{Specifics}\\ \midrule
     \citep{fomicheva-2021,fomicheva-2021b} & FI & L & A+S & Various & Plausibility \\\midrule
     \citep{chen-2021} & FI & L & A & Perturbations & Faithfulness \\\midrule
     \citep{yuan-2021} & TBD & L & A & TBD & Plausibility \\\midrule
     Adversarial Attacks & EbE & L & A & Perturbations & -\\\midrule
     \citep{kaster-2021} & EbS/CA & G & A & TBD & Faithfulness\\\midrule
     \citep{sai-2021} & CA & G & A & Perturbations & TBD\\
     \bottomrule
\end{tabular}
\caption{Explainability for MT metrics. The types are Concept Attribution (CA), Feature Importance (FI), Explanation by Example (EbE) and Explanation by Simplification (EbS). L/G considers Local (L) vs Global (G) and A/S considers Agnostic(A) vs Specific(S). The "Eval" column indicates whether the authors evaluated with respect to plausibility and/or faithfulness. The column ``Goals'' specifies, which of the goals of section \ref{} can be addressed with the respective techniques. Thereby, we consider (B)ias detection, metric (D)iagnosis and metric (E)xpressiveness. Lastly, "Challenges" shows which of the properties \textit{(m)ultilingual input, varying (s)cales, (n)umeric output, relation to translation (e)rrors and interdependent (p)airwise input} are being addressed.}
\label{taxonomy}
\end{table*}

==> legacy/old_structure/4_localTech.tex <==
\section{Local Techniques}
As described in the previous section, local explainability techniques provide additional information that helps (certain audiences) to understand model behaviour with specific input/output pairs. In this section we introduce recent works that investigate local techniques to explain MT metrics or related setups. Additionally, we conduct preliminary experiments on explaining metrics with adversarial samples. We structure the section based on the output type of the methods. 

\subsection{Word-Level Feature Importance Explanations}
In the last section we detailed feature importance explanations, i.e. explanations that assign each input feature an importance score with respect to a specific output. For textual input, these features are often assigned on a word- or subword-level. 

The following two works consider the local explainability of reference-free machine translation evaluation. When humans evaluate translations, they often focus on the errors that they can identify on a word- or phrase-level \citep{freitag-2021}. \citet{fomicheva-2021} and the 2021 Eval4NLP shared task \citep{fomicheva-2021b} build on this idea and evaluate how well feature importance is correlated with human word-level error annotations. They show that, on one hand, this can enable to leverage strong sentence-level metrics on a word-level. On the other hand, the correlation could be used as an indicator of plausibility (see section \ref{Plausibility}), as the correlation to the human measure of correctness of a sentence, word-level errors, is used. I.e. word-level error extraction from sentence-level metrics could be used as additional benchmark for explainability methods. \citet{fomicheva-2021} explore this approach with the strong reference-free metric Transquest \citep{ranasinghe-2020}. They perform experiments on the MLQE-PE corpus \citep{fomicheva-2020} (see section \ref{datasets}). In specific, \citet{fomicheva-2021} leverage the hypothesis tags and compare them with feature importance scores. The tags in MLQE-PE also contain annotations for the gaps between words. These are dropped in their case. They label correct words with 0 and incorrect words with 1. As feature importance scores are continuous rather than binary, they use the metrics \textit{area under the receiver operator characteristic curve} (AUC), \textit{average precision} (AP), \textit{recall at top-k} (R@K) and \textit{accuracy at 1} (A@1). 

\citet{fomicheva-2021b} choose four well-known explainability techniques in order to extract the feature importance scores. They use \textit{LIME} \citep{ribeiro-2016} as exemplary model-agnostic technique. For each sample (source and/or hypothesis) that is explained, LIME produces a ``dataset'' of perturbations by dropping or replacing words at random and evaluates its metric scores. This ``dataset'' is used to train a linear model to behave similar as the original metric for the given sample. Sentences with less perturbations are weighted higher, as LIME has the goal to approximate the original metric around the sample. Further, \citet{fomicheva-2021b} choose three model-specific approaches for neural networks: information bottleneck \citep{schulz-2020}, integrated gradients \citep{sundararajan-2017} and attention \citep[e.g.][]{wiegreffe-2019, serrano-2019}. Note that attention is even more specific to certain architectures such as transformers \citep{vaswani-2017}. Information bottleneck determines feature importance scores by testing, which features can be disturbed the most by injecting noise at an intermediate layer with only minimal changes to the original prediction. The integrated gradients method first requires a baseline, e.g. a tensor of zeroes. Then it replaces the hidden states at a given layer with this tensor and follows the computation of partial derivatives of the output with respect to the input. The same computation is repeated for all tensors along a linear path from baseline to original input and the results are summed. Finally, \citet{fomicheva-2021b} use self-attention for feature importance by averaging weights across attention heads. Attention has seen wide but controversial use for explainability \citep{bastings-2020}. Additionally, \citet{fomicheva-2021b} compare a metric that was trained with supervision to compute word-level errors in a classification setting \citep{ranasinghe-2021} and a glass-box approach that uses the word-level translation probabilities of each word of the known MT model as feature importance \citep{fomicheva-2020b}. They report the following key findings:
\begin{itemize}
    \item LIME performs worse than the other methods, which is attributed to the fact that LIME works with perturbations of the input rather than at a hidden state. Hence, the context is not established for LIME (TODO: Is this really the case?).
    \item Feature importance for word-level explanation performs competitive to the glass-box approach and integrated gradients even approaches the performance of the supervised metric.
    \item The explained metric seems to only take the source into account in later layers. Likewise, explainability techniques that leveraged these layers performed best.
    \item Later layers of the metric assign a high importance to frequent words in high-quality translations and a high importance to less frequent words in low-quality translations. This implies that errors are more important in low-quality settings. (TODO: Did I understand this correctly?)
\end{itemize}

\label{eval4nlp}
The 2021 Eval4NLP \citep{fomicheva-2021} shared task explores this evaluation approach of plausibility and comprises a competition for the highest AUC, AP and R@K scores for source and hypothesis word-level error annotations. For training and development, they provide extracts from MLQE-PE. However, as test-set they provide a new dataset that contains directly annotated word-level labels (see section \ref{eval4nlpdata}). As baseline systems, the organizers provide a random baseline, as well as Transquest explained with the model-agnostic LIME and XMoverscore \citep{zhao-2020} explained with the model-agnostic SHAP \citep{sundararajan-2017}. Seven systems were submitted to the shared task, three of which leveraged word-level supervision. One system with synthetic data \citep{rubino-2021} and two with manually annotated data \citep{treviso-2021,polak-2021}. Overall, the system that leveraged synthetic data performed best on three out of four language pairs. They obtain word- and multiple sentence-level scores from the alignment of pseudo-references (MT translations of the source) and references on parallel corpora using reference-based metrics. With these, they jointly fine-tune the XLMR \citep{conneau-2020} language model. To calculate the influence of the metrics, they propose to learn the distinction of each metric in additional parallel layers (metric embeddings), all of which are connected via attention. Word-level scores are extracted from this attention component. The best system that doesn't use word-level supervision leverages L2-normalized attention weights to extract word-level scores \citep{treviso-2021}. In general, multiple works have explored a broader array of explainability techniques and it seems that attention based methods beat gradient-based methods and perturbation-based methods perform worst. 

A potential issue with this evaluation approach is that it does not consider the property of faithfulness (see section \ref{Faithfulness}). Hence, there is no guarantee, that the extracted word-level scores actually reflect the sentence-level score. When used as a benchmark for explainability, a word-level metric might be employed as explainability technique and achieve good results without taking a look at the underlying metric. For future work we suggest to provide accompanying faithfulness evaluations.

As part of this paper\todo{MF: This is unpublished work, right? If so, this should be presented in much more detail, maybe in a separate section}, we provide results for four additional pairs of metric + explainability technique, which we will refer to as \textit{hard reference-free metrics}. Hard metrics like BLEU and METEOR are interpretable and reference-based. Besides using explainability techniques, word-level scores could be computed from them directly. Here we explore, how well the word-level scores extracted from these metrics perform on the shared task. In order to do so, we obtain pseudo references using 1. a SOTA MT model and 2. word by word (wbw) translations using a dictionary obtained with Google Translate \footnote{\url{https://translate.google.com/?hl=de}}. Further, we use SHAP \citep{sundararajan-2017} to extract word-level scores. Table \ref{tab:HardRefFree} shows the results on the test sets compared with the baselines of the shared task. The results are unexpected, as the hard reference-free metrics outperform the baselines in many dimensions. Even with word-by-word translations the approach outperforms the baselines for AUC. This finding suggests that due to the interpretability of METEOR, SHAP is able to extract better feature importance scores than from e.g. XMoverScore. 

 \begin{table}
\centering
\begin{tabular}{|l|ccc|c|} \hline
     & \multicolumn{3}{c|}{Hypothesis} & \multicolumn{1}{c|}{} \\
    \textbf{System} & AUC & AP & RtopK & Pearson\\\hline
TranslationBLEU$_{full}$ + SHAP|et-en & \textbf{0.754} & 0.541 & 0.418 & 0.482 \\
TranslationMETEOR$_{full}$ + SHAP|et-en & \textbf{0.754} & \textbf{0.562} & \textbf{0.444} & 0.581 \\
TranslationMETEOR$_{wbw}$ + SHAP|et-en & 0.67 & 0.445 & 0.323 & 0.318 \\
Transquest+LIME (Baseline)|et-en & 0.624 & 0.536 & 0.424 & \textbf{0.772}\\
XMoverScore+SHAP (Baseline)|et-en & 0.616 & 0.441 & 0.338 & 0.494\\\hline
TranslationBLEU$_{full}$ + SHAP|ro-en & \textbf{0.831} & 0.592 & 0.446 & 0.562 \\
TranslationMETEOR$_{full}$ + SHAP|ro-en & 0.826 & \textbf{0.603} & \textbf{0.458} & 0.701 \\
TranslationMETEOR$_{wbw}$ + SHAP|ro-en & 0.752 & 0.493 & 0.342 & 0.397 \\
Transquest+LIME (Baseline)|ro-en & 0.634 & 0.523 & 0.415  & \textbf{0.899}\\
XMoverScore+SHAP (Baseline)|ro-en & 0.666 & 0.438 & 0.295  & 0.695\\\hline
TranslationBLEU$_{full}$ + SHAP|ru-de & 0.795 & 0.525 & 0.420 & 0.490 \\
TranslationMETEOR$_{full}$ + SHAP|ru-de & \textbf{0.806} & \textbf{0.546} & \textbf{0.435} & \textbf{0.597} \\
TranslationMETEOR$_{wbw}$ + SHAP|ru-de & 0.679 & 0.399 & 0.288 & 0.273 \\
Transquest+LIME (Baseline)|ru-de & 0.545 & 0.334 & 0.220 & 0.505\\
XMoverScore+SHAP (Baseline)|ru-de & 0.460 & 0.271 & 0.145 & 0.335\\\hline
TranslationBLEU$_{full}$ + SHAP|de-zh & 0.633 & 0.391 & 0.261 & 0.275 \\
TranslationMETEOR$_{full}$ + SHAP|de-zh & \textbf{0.647} & \textbf{0.420} & \textbf{0.294} & 0.376\\
TranslationMETEOR$_{wbw}$ + SHAP|de-zh & \textbf{0.617} & \textbf{0.390} & \textbf{0.273} & 0.222\\
Transquest+LIME (Baseline)|de-zh & 0.404 & 0.262 & 0.164 & \textbf{0.489}\\
XMoverScore+SHAP (Baseline)|de-zh & 0.522 & 0.328 & 0.227 & 0.252\\
\hline
\end{tabular}
\caption{Performance of ``hard reference-free metrics'' on the Eval4NLP shared task. Metric$_{full}$ indicates that a full translated sentence was used as pseudo-reference. Metric$_{wbw}$ indicates that the word by word translated source was used as pseudo-reference. Bold values indicate the best score per column and language pair.}
\label{tab:HardRefFree}
\end{table}

\subsection{Sentence-Pair Feature Importance}
With GMASK, \citet{chen-2021} introduce an explainability technique that provides hierchical feature attributions on sentence pairs. I.e. the technique forms groups of words between two input sentences and assigns each group an importance score. This approach is especially fitting to explain MT metrics, as these are based on sentence pairs in most cases. For example, when one word in a source is translated into multiple words in the hypothesis, GMASK can identify this connection and provides joint importance values. In specific, the method seeks to fulfill three core properties: (1) providing correct importance selections, (2) only consider the most relevant words, (3) correlated words are masked together. GMASK learns binary masks that indicate for each embedding in the two input sentences, whether it should be dropped or kept. Thereby, it tries to keep the originally predicted output while reducing the number of relevant words. 

\citet{chen-2021}\todo{MF: Can we run some quick experiment to apply their work to MT evaluation?} evaluate their approach on a dataset for natural language inference and three datasets for paraphrase identification. To evaluate faithfulness, they apply the AOPC score discussed above. Further they determine post-hoc accuracy (see section \ref{Faithfulness}) and check how well the top predictions indicate the original outcome. This could be reasonable in their classification setup, but is problematic with metrics (e.g. due to the ood problem). Further they employ a degradation test \citep[e.g.][]{schulz-2020}. Overall, their results indicate that their method is the most faithful compared to LIME, L2X, IBA and IMASK.

For metrics, properties that are specific to classification, such as keeping the original classification result, would need to be adapted to their numeric output types. For example, by using intervals that represent classes.
%GMASK learns a set of binary word masks \textbf{W} where each is applied to x and y via element-wise multiplication. Hence, mask positions with 0 will mask out the respective words.

%Let $x=(x_1^T,...,x_n^T)^T$ and $y=(y_1^T,...,y_n^T)^T$ be the sentences with word embeddings $x_i,y_i \in \R^d$ and $f(x,y)$ be a metric.

\subsection{Generation Direction}
The recently proposed metric BARTScore by \citet{yuan-2021} treats NLG evaluation as a generation task. They use BART \citep{lewis-2020} for text generation to predict the probability of a sentence to be generated given another sentence. The resulting probability is used as metric score. The sentence-probability is computed as a sum of token-level log-probabilities:
$$\text{BARTScore} = \sum^m_{t=1}\omega_t\log p(y_t|y<t,x,\Theta)$$
Here, $\omega$ is a placeholder for idf-weighting, that is not applied in the BARTScore paper. The token level probability of a token $y_t$ is determined given the previous target-tokens $y<t$, the source input $x$ and a BARTModel with parameters $\Theta$. I.e. the same setup as when training a translation model with teacher-forcing is used.
\citet{fomicheva-2020b} follow a similar idea in the domain of quality estimation. They use the confidence of the model that produced the hypothesis itself as quality-estimation score, rather than using an external one. \citet{yuan-2021} evaluate different generation directions: Faithfulness: SRC->HYP, Precision: REF->HYP, Recall: HYP->REF, F-Score: HYP<->REF (the arithmetic average of precision and recall). For example, for SRC->HYP the metric score is the probability that BART generates the HYP given the SRC. They evaluate the metric in the context of machine translation evaluation and data-to-text generation, where they use the F-Score. Further, they evaluate summarization tasks with varying directions. It is stated that these directions would encapsulate different evaluation perspectives. E.g. HYP->REF would encapsulate \textit{semantic coverage}, i.e. how well the meaning of the reference is captured by the hypothesis. As such, providing the results of different generation directions can be treated as explainability approach that provides additional information on a sample.

Using multilingual translation models such as mBART \citep{liu-2020} or m2m100 \citep{fan-2020}, BARTScore can be easily adapted for further domains such as reference-free machine translation evaluation. In the MT domain it is similar to the metric PRISM \citep{thompson-2020}, which employs a custom multilingual MT model to determine the probability for a translation (or cross-lingual paraphrasation). These metrics can inherently provide word-level feature importance scores (see section \ref{sec:dimensions}) by interpreting the token level translation probabilities as importance. As an example, we compare a reference-free ``BARTScore'' using m2m100 (M2MScore) with Transquest+Shap in table \ref{tab:M2MScore}.\todo{MF: What is our conclusion here? Also, for Eval4NLP we should compare not only with baselines but also with the best performing approach, I think}

\begin{table}[ht]
\centering
\begin{tabular}{|l|ccc|ccc|c|} \hline
     & \multicolumn{3}{c|}{Hypothesis} & \multicolumn{3}{c|}{Source} & \multicolumn{1}{c|}{} \\
    \textbf{System} & AUC & AP & RtopK & AUC & AP & RtopK & Pearson\\\hline
M2MScore | et-en & \textbf{0.751} & \textbf{0.597} & \textbf{0.494} & \textbf{0.774} & \textbf{0.566} & \textbf{0.401} & \textbf{0.783} \\Transquest+LIME | et-en & 0.624 & 0.536 & 0.424 & 0.544 & 0.440 & 0.309 & 0.772\\\hline
M2MScore | ro-en & \textbf{0.837} & \textbf{0.658} & \textbf{0.509} & \textbf{0.771} & \textbf{0.513} & \textbf{0.356} & 0.843 \\Transquest+LIME | ro-en & 0.634 & 0.523 & 0.415 & 0.478 & 0.351 & 0.243 & \textbf{0.899}\\\hline
M2MScore | ru-de & \textbf{0.755} & \textbf{0.532} & \textbf{0.418} & \textbf{0.682} & \textbf{0.497} & \textbf{0.402} & \textbf{0.685} \\Transquest+LIME | ru-de & 0.545 & 0.334 & 0.220 & 0.474 & 0.287 & 0.159 & 0.505\\
\hline
M2MScore | de-zh & \textbf{0.597} & \textbf{0.378} & \textbf{0.254} & \textbf{0.539} & 0.349 & 0.216 & 0.192\\
Transquest+LIME | de-zh & 0.404 & 0.262 & 0.164 & 0.534 & \textbf{0.427} & \textbf{0.320} & \textbf{0.489}\\\hline
\end{tabular}
\caption{Results of M2MScore on the test sets of the Eval4NLP shared task. Transquest+LIME is a baseline provided by the organizers.}
\label{tab:M2MScore}
\end{table}

Based on the evaluation directions presented by \citep{yuan-2021}, the recent ExplainaBoard webtool, provides a possibility to compare and benchmark evaluation metrics. This dimension is provided under the title ``Meta Evaluation for Automated Metrics''. 


\subsection{Chunk Alignment}
The approaches we have described up to this point leverage numerical explanations. While these give an insight into properties of the explained samples, textual explanations might be easier to comprehend for non-experts and therefore further support the goal of accessible metrics. The second tasks of SemEval-2015 \citep{agirre-2015} and -2016 \citep{agirre-2016} explore this setting and ask participants to perform a labelled chunk alignment between two sentences as explanation for semantic textual similarity. In the respective datasets, they annotate how phrases relate between sentences and assign scores to the relation strength based on a 0 to 5 scale, where 0 indicates unrelatedness. As example, the authors consider the sentences ``12 killed in bus accident in Pakistan'' and ``10 killed in road accident in NW Pakistan''. They show sample alignments for ``[12] <==> [10]'' to be similar with a relation strength of 4 and ``[in bus accident] <==> [in road accident]'' to be a specification with relation strength of 4. The annotation process first assigns chunks, then scores and then the label(s). The relationship is chosen from predefined labels, where 0 is always assigned NIL and 5 means equivalence. To measure the system quality, they use different F1 measures taking into account the scores, the labels and both. Their baseline system uses rules to assign the label. The best performing system at that time used a multi layer perceptron and multi-task learning \citep{magnolini-2016}. There are recent works that improve on the task, especially the phrase level alignment. For example \citet{lan-2021, arase-2020} provide new datasets and approaches for this topic. 

\subsection{Adversarial Samples}
\todo{MF: I think this approach is very interesting and different from everything discussed above. It probably deserves a separate section and should be mentioned in the introduction as one of the contributions of the paper (if this is unpublished work).}\citet{szegedy-2014, goodfellow-2015} show that neural networks can be susceptible to adversarial attacks. This term describes the perturbation of input to machine learning models, such that their output changes, but the input remains close to the original from a human's perspective. In object recognition for example, inputs can be augmented with noise that is imperceivable for humans but leads to different prediction outcomes \citep{szegedy-2014, goodfellow-2015}. In NLP we can differentiate between sentence-level, word-level and character-level attacks. Interestingly, sentence- and word-level attacks often have the goal to produce examples that appear similar in terms of meaning, while character-level attacks often aim to produce examples that are visually similar \citep{eger-2019}. While changes to characters can go unnoticed, changes to words or sentences are easier to recognize. 
Following the notion that knowing a model's failure cases can help in improving the model, adversarial attacks are interwoven with explainability \citep{linardatos-2021}. Presenting single adversarial examples, could be interpreted as a local explanation-by-example technique. As these samples only introduce small changes, they also lie in a neighbourhood of the original sample (as for example leveraged by LIME). However, finding the key difference to the original input remains to human reasoning or further pipeline steps. It is to note that, if the changes were actually imperceivable to a human, they could not provide local explanations. I.e. ideally, we search for attacks that produce paraphrases that keep the meaning and change the metric score.
\todo{YG: two problems here: i) the paragraph is too long; ii) we need to split existing methods from our proposed method. I'm wondering whether we should put our proposed method to a different section.} \PL{I agree with YG. We should write our contributions apart from surveys in separate sections.}
Figure \ref{advDesign} shows our design of this approach. An adversarial attacker takes the original input of a metric and perturbs it to generate an adversarial hypothesis HYP$^*$. The metric then computes another score for the adversarial example. The attack is successful if this adversarial score is as different to the original score as possible and the perturbed hypothesis is as similar to the original hypothesis as possible. 
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{images/AdversarialMTE.JPG}
    \caption{Adversarial Attacks on Machine Translation Evaluation Metrics} \label{advDesign}
\end{figure}
To maximize the difference between the original score and the adversarial score, we can for example maximize their mean squared error. However, minimizing the distance between the two hypotheses is problematic. This is a comparison of a pair of two strings. Therefore, metrics that measure their similarity could be used. On the other hand, these are exactly the type of metric that is being attacked with this setup. I.e., the successfulness of an attack on a metric would be evaluated with the same type of metric. Hence, when the similarity metric that checks the validity of the adversarial example is susceptible to the same attacks as the metric that is attacked, these attacks would not be identified. Likewise, if an adversarial example is only a failure case of the similarity metric, but not of the attacked metric, adversarial examples might falsely be flagged as valid. \citet{morris-2020} explores the second case under the name \textit{second order adversarial attacks}. As an example, assume we attack BERTScore and validate the similarity of the generated hypotheses with BLEU. Then second order adversarial attacks would attack BLEU to falsely indicate similarity while the difference of the output scores of BERTScore is still maximized. 

Most word- and sentence- level adversarial attacks consider a classification setting. To apply them to metrics, we discretize the metric score into classes following a three step process. First, we select a dataset and calculate a metric score for each sample and metric. Second, we determine $k$ quantiles for each metric's scores, where $k$ is the number of classes we want to discretize to. Third, for each class of interest, we filter the metric scores for samples that lie in the same class for all metrics. Class probabilities are based on the procentual distance to the centre of the class intervals the metric score lies in between.

We apply the following adversarial attacks to the discretized scores:
\begin{itemize}
    \item \textbf{BERT-Attack} \citep{li-2020} leverages BERT \citep{devlin-2019} for word replacement in a word-level adversarial attack. First it ranks tokens based on their importance for the original prediction (here the metric score) using feature importance explanations. Then the tokens are iterated in order of this ranking. For each token, k replacement candidates are checked and if they are not successful, the next token in the importance ranking is assessed. If the token is a word, it is replaced with one of the top-k replacement candidates obtained by feeding the sentence to BERT (without usage of a mask). If the token is a sub-word, the other sub-word tokens that belong to the word are identified, all possible sub-word combinations are listed and their probabilities to occur as a word replacement are determined with BERT. Each replacement is evaluated with respect to the goal of the attack. Once the original prediction changes, the attack is successful. 
    \item \textbf{Textfooler} \citep{jin-2020} also ranks the words for their importance. The ranked words are iterated and for each word k replacement candidates are tested. The candidates are determined as the top-k words that have the same POS-tag and a high cosine-similarity of their static word-embeddings. Further, only candidates that keep the universal sentence encoder (USE) \citep{cer-2018} similarity of the perturbed sentence to the original sentence higher than a threshold are considered. If the predicted class doesn't change after checking all candidates for a word, the candidate that minimized the predicted class probability is kept and the next important word is perturbed. 
    \item \textbf{Textfooler-Adjusted} \citep{morris-2020-reeval} adds further constraints to textfooler. It sets higher thresholds on minimal word- and sentence-level similarity (based on static word embeddings and USE). Additionally, it employs Language-Tool \citet{naber-2003} to impose a constraint on the number of errors introduced by an attack.
    \item \textbf{SCPN} \citep{iyyer-2018}, or syntactically controlled paraphrase networks, are a technique to generate paraphrasations of an input sentence that follow a given syntactic parse tree. The setup consists of two components. A \textit{parse generator} learns to generate parse trees from parse templates and a paraphrase generator paraphrases sentences based on the \textit{parse tree}. The parse generator is necessary as parse templates are easier to specify for human users. To interpret the paraphrased sentences as adversarial examples, \citet{iyyer-2018} select the 20 most frequent parse templates in a corpus and use these to paraphrase each sentence in their test setup. Next, they apply constraints to encourage similarity to the original parse tree. Therefore, they use n-gram overlap and similarity of sentence embeddings. The SCPN is used for adversarial attacks by iterating the generated paraphrases as replacement.
    \item \textbf{Word-level Hotflip} \citep{ebrahimi-2018} uses the gradients of one-hot encoded words with respect to a prediction to determine the importance of the words. They then replace it with other words that have embeddings with a high cosine similarity to the original word's, have the same part of speech tags and are no stop-words.
\end{itemize}

We use TextAttack \citep{morris-2020-textattack} and OpenAttack \citep{zeng-2020} as frameworks. The described attacks originally are untargeted, i.e. they follow the goal of changing the resulting class. Here, we use a targeted setup for BERT-Attack, Textooler and Textfooler-Adjusted, by leveraging the respective class of Textattack. 

In figure \ref{fig:advattackExample} we show an adversarial sample for a de-en (German-English) sentence from the dataset used in the WMT20 metrics shared task. In the example, we use 5 classes. The number on the left indicates the original prediction, the number on the right indicates the changed class. For example, BERT-Attack changed the prediction of BLEU from class 4 to 0 by inserting the word \textit{terrified} instead of \textit{Frightened}. When a metric is missing, the attack was not successful for this combination. Interestingly, only BERT-Attack and Textfooler-Adjusted seem to find perturbations that keep the meaning of the original translation. We note that the source sentence is ungrammatical, which might confuse the metrics. Using the highlighted words as explanations, we could see that BLEU and Transquest graded other reasonable translations lower and hence distrust them in this case. BLEURT on the other hand was not attacked with a reasonable permutation, therefore we have more confidence it produced a good translation. For longer sentences however, it might become too difficult to reason about these changes. Another interesting finding is that many of the attacks were flagged as successful, even though they don't keep the meaning. This problem was investigated in recent work by \citet{morris-2020-reeval,hauser-2021}. By performing a human evaluation of adversarial attacks, they find that many attacks perform weakly. To better judge the quality of an adversarial sample, they introduce checks for grammaticality and semantic similarity.

\begin{figure}
  \centering
    \includegraphics[width=0.6\textwidth]{images/AdversarialAttackTextExample.PNG}
    \caption{Exemplary attacks on a sample from WMT20}
    \label{fig:advattackExample}
 \end{figure}

We also apply attacks to a subset of the zh-en (Chinese-English) dataset of WMT20. Thereby, we divide the scores into 3 classes and filter for all samples that each considered metric places in the same class. Improving translations is a difficult task compared to making them worse, hence we investigate the change from the highest class to the lowest class. 653 samples have been placed in the highest class. Further, we only apply BERT-Attack, Textfooler and Textfooler-Adjusted. Figure \ref{fig:sr653} shows the success rate of the attacks per metric. An intriguing finding is that BERT-Attack and Textfooler are performing very well against supervised metrics, have a smaller success on metrics that are based on word-level similarities such as XMoverscore and BERTScore and are least successful for hard metrics. Intuitively it makes sense for these metrics to be more robust, as they are based on word-level results that need bigger changes to perturb. We follow \citet{morris-2020-reeval} and show the respective perturbation rates (figure \ref{fig:sim653}), the number of new grammatical errors introduced (figure \ref{fig:ge653}) and the sentence similarity before and after perturbation (figure \ref{fig:smi653}). The black tiles indicate that no successful attack was found. The perturbation rates show that the attacks need less perturbations to attack the supervised metrics, more perturbations for soft matching metrics like XMoverScore and MoverScore and the most perturbations for hard metrics. For Textfooler-Adjusted the distinction is not that strong, but the number of samples identified by this attack is so low that the results might be by chance. Similarly to the previous finding, less grammatical errors are introduced to attack supervised metrics and the semantic similarity can be kept on a higher level. Also, it is to note that the constraints of Textfooler-Adjusted work, such that no new grammatical errors are introduced and the semantic similarity stays the highest. \citet{morris-2020-reeval} highlight, that the respective constraints make it difficult to compare the results of the attacks directly. Still, it is possible to say that, using the standard constraints of the attacks, BERT-Attack on average introduces more grammatical errors than Textfooler. At the same time, they have comparable sentence similarities. In terms of explainability, these insights could be interpreted as global explanations. The adversarial attacker could be seen as an explainer that provides additional insights about a metric. Thereby, it helps with the goal of further improving the metrics.
 
 \begin{figure}
  \centering
    \includegraphics[width=\textwidth]{images/rerun_success.png}
    \caption{Success rate of adversarial attacks on 653 zh-en samples from WMT20}
    \label{fig:sr653}
 \end{figure}

 \begin{figure}
  \centering
    \includegraphics[width=\textwidth]{images/rerun_pert_rate.png}
    \caption{Perturbation rate of adversarial attacks on 653 zh-en samples from WMT20}
    \label{fig:sim653}
 \end{figure}
 
 \begin{figure}
  \centering
    \includegraphics[width=\textwidth]{images/rerun_gram_error_rate.png}
    \caption{Avg. grammatical error introduced by adversarial attacks on 653 zh-en samples from WMT20}
    \label{fig:ge653}
 \end{figure}
 
 \begin{figure}
  \centering
    \includegraphics[width=\textwidth]{images/rerun_sem_sim.png}
    \caption{Average sentence similarity of the original and perturbed hypothesis on 653 zh-en samples from WMT20}
    \label{fig:smi653}
 \end{figure}

To summarize, we have shown how adversarial attacks can be applied to MT metrics. Further, we have discussed, to what extend they provide local and global explanations. Our results indicate that supervised metrics like COMET or BLEURT are the most susceptible and might benefit from adversarial training.

Where \citet{sai-2021} find model failure cases by applying perturbation templates (see section \ref{sec:pertChecklist}), we take a different approach and apply adversarial attacks to identify the general robustness of evaluation metrics as well as single failure cases. Their approach has the benefit of providing a more fine-grained overview, which kind of perturbations cannot be handled by a metric. Using adversarial attacks on the other hand allows to consider a broader spectrum of perturbations showcasing to which extend metrics can fail in worst-case scenarios. Our approach could be extended to provide more fine-grained results by providing another model that checks which type of perturbation was introduced by the adversarial sample.

\subsection{Inverse Metrics}
\label{InverseMetrics}
Adversarial attacks are required to produce examples that lie as close to the original input as possible. We argue that the property, which makes them interesting for local explanations is that the change can still be perceived. For an explanation, it might not be necessary to be close to the original sentence. To that end, we introduce \textit{inverse metrics}, which can be interpreted as a special form of adversarial attacks or counterfactual examples. A similar approach can be found in Computer Vision, where CNNs are explained by inverting their computation \citep{mahendran-2014}. We define an inverse metric METRIC$^{-1}$ as follows:
$$\text{METRIC}^{-1}(\text{SRC|REF},\text{score})=\text{HYP*}\longleftrightarrow\text{METRIC}(\text{SRC|REF},\text{HYP*})=\text{score}$$
In other words, the inverse metric returns a hypothesis for which the metric will return a given score. If a good reference-free machine translation evaluation metric assigns a score of 1 to a perfect translation of a source, the inverse metric of the source and the score 1 should ideally return a perfect translation as well. If the lowest possible score is 0, the inverse metric of the source and the score 0 should return a translation that is as bad as possible (as measured by the metric).
Note that the output of an inverse metric could be interpreted as a targeted, unconstrained adversarial attack on metrics with numeric outputs, or, depending on the definition, as counterfactual. The only exception is, when the target score is equal or similar to the original score. Here, the output could be viewed as prototypical example for a score. Figure \ref{counterfactualExplanation} displays a hypothetical example of how such examples can provide insights into a model's local behaviour. By sampling other hypotheses around the original score, it could be shown what the metric indicates as better or worse than the original hypothesis. In case of metrics with a good performance this could be used to improve translations. In case of weak metrics, it could show the failure cases of the metric, e.g. if the inverse metric finds hypotheses that are grammatically worse but get higher scores. 
\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{images/CounterfactualExplanation.png}
    \caption{Hypothetical examples around a given hypothesis} \label{counterfactualExplanation}
\end{figure}

Figure \ref{fig:inversealgres} shows example neighbourhoods we queried for BLEU and BLEURT. We used a technique that iteratively perturbs words based on mask replacement, to find an input that results in a score as close the desired target output as possible (see Appendix \ref{sec:InverseTech}). Based on these results, we can verify that BLEU does not try to preserve semantics. Further, for BLEURT we acquire a rather interesting improvement ``My cat dates back two generations .''. While being close in meaning, it is not a phrase that would be used in natural language. As the technique produces a neighbourhood for a sample, it might also be integrated into other explainability techniques such as LIME.

\begin{figure}
  \begin{subfigure}[b]{0.9\textwidth}
    \includegraphics[width=\textwidth]{images/InverseMetricBleu.PNG}
    \caption{BLEU}
    \label{fig:inversealgres1}
  \end{subfigure}
  \hfill\\
  \begin{subfigure}[b]{0.9\textwidth}
    \includegraphics[width=\textwidth]{images/InverseMetricBLEURT.PNG}
    \caption{BLEURT}
    \label{fig:inversealgres2}
  \end{subfigure}
  \caption{Exemplary hypothesis neighborhood}
  \label{fig:inversealgres}
\end{figure}


==> legacy/old_structure/5_globalTech.tex <==
\section{Global Techniques}
As discussed in the previous sections, most explainability techniques for neural networks consider local explanations. While these can provide an insight into a model's decision process for specific samples, often it also is desireable to characterize how the model will behave in general. In this section we consider recent approaches of global explainability.

\subsection{Disentanglement along Linguistic Factors}
\label{globalExpPaper}
\citet{kaster-2021} propose a global explainability technique that decomposes the score of segment-level BERT-based metrics into different linguistic factors. In specific, they explore the degree to which metrics consider each of the properties \textit{syntax}, \textit{semantics}, \textit{morphology} and \textit{lexical overlap}. As a first step, they use the following methods to determine ``ground truth'' scores for the influence (similarity) each of the properties should have:
\begin{itemize}
    \item \textbf{Lexical Overlap Score (LEX):} The lexical overlap score is determined using BLEU \citep{papineni-2002} with unigrams. This follows the intention that word order should be ignored for lexical overlap. For reference-free metrics they generate pseudo-references by translating the source sentences with Google Translate before applying BLEU.
    \item \textbf{Morphological Score (MOR):} The morphological score computes the cosine similarity of morphologically enriched sentence embeddings. These are based on word embeddings that were finetuned on morphological lexicons following \citet{faruqui-2015}.
    \item \textbf{Semantic Score (SEM):} The semantic score leverages human annotated sentence level scores provided with different datasets for the evaluation of machine translation evaluation metrics.
    \item \textbf{Syntactic Score (SYN):} The syntactic score measures the syntactic similarity between hypothesis and source/reference with the tree edit distance (TED) \citep{bille-2005} of parse trees generated by the Stanford dependency parser \citep{chen-2014}.
\end{itemize}
\citet{kaster-2021} z-score all scores in order to make them comparable. Table \ref{table:example} shows an example they use to demonstrate the different scores for two sentence pairs. 

\begin{table*}[!htb]
\small 
\centering
\begin{tabular}{p{4.8cm}|p{4.8cm}|cccc}
     \toprule
     \textbf{Hypothesis} ($y$) & \textbf{Reference}/\textbf{Source} ($x$) & \textbf{SEM} & \textbf{SYN} & \textbf{LEX} & \textbf{MOR}\\ \midrule
     It is a boy , likes to sport , but it cannot do it because of their very. & He is a boy, he likes sports but he can't take part because of his knee. &  -1.57  & 0.98 & -0.59 & -0.87 \\ \midrule
     
     Zwei Besatzungsmitglieder galten als vermisst.	 & Two crew members were regarded as missing.  &	0.83 & 0.99  & 0.46 & -2.40\\
     \bottomrule
\end{tabular}
\caption{Example setups with normalized semantic, syntactic, lexical overlap and morphological scores \citep{kaster-2021}.}
\label{table:example}
\end{table*}

To explain metrics in terms of these properties, \citet{kaster-2021} determine SEM, SYN, LEX and MOR for all sentence-pairs in a dataset. Further they score each sentence-pair with the metric that should be explained. Based on these, they estimate the following linear regression:
$$m(x,y)=\alpha*sem(x,y)+\beta*syn(x,y)+\gamma*lex(x,y)+\delta*mor(x,y)+\eta$$
$x$ is a reference or source sentence, $y$ is a hypothesis sentence and $sem$, $syn$, $lex$ and $mor$ are the scores of the respective linguistic properties. $m$ is the metric that is explained, $\eta$ is an error term and $\alpha$, $\beta$, $\gamma$ and $\delta$ are learned weights that indicate the linear influence each property has on the metric score. The degree to which the learned regressors approximate the metric function is determined with the determination coefficient $R^2$:

$$R^2=1-\frac{\sum_i(y_i-\hat{y}_i)^2}{\sum_i(y_i-\bar{y})^2}$$

For a sentence $i$, $y_i$ is the original metric score and $\hat{y}_i$ is the value predicted by the regression. $\bar{y}$ is the mean of the original metric scores. I.e., $R^2$ is the inverse of the sum of squared distances divided by the sum of squared totals. Its value gets smaller, when the results of the learned function diverge from the original metric score, while the metric score is not an outlier of the metric.

\citet{kaster-2021} conduct experiments with the reference-based metrics BERTScore \citep{sellam-2020}, MoverScore \citep{zhao-2019}, SBERT \citep{reimers-2019}, SBERT-WK \citep{wang-2020b} and BLEURT \citep{sellam-2020}. Further, they consider the reference-free metrics mSBERT \citep{reimers-2020}, MUSE \citep{yang-2020b}, LaBSE \citep{feng-2020}, LASER \citep{artetxe-2019} and XMoverScore \citep{zhao-2020}. Thereby, SBERT, SBERT-WK, mSBERT, MUSE, LaBSE and LASER transformer models are used to compute sentence embeddings of which sentence similarity is computed using cosine similarity. They also apply reference-free metrics to the reference-based case. They conduct experiments with data from WMT15-WMT17 \citep{stanojevic-2015,bojar-2016,bojar-2017} for the domain of machine translation and STSB \citep{cer-2017} for the domain of semantic text similarity. The following key findings are reported:
\begin{itemize}
    \item The $R^2$ value is generally higher for reference-based metrics than for reference-free metrics. I.e. the learned regression can better approximate reference-based metrics. \citet{kaster-2021} hypothesize that this is due to a missalignment between languages in multilingual embeddings. They introduce a fifth property \textit{cross-lingual bias} whose ``ground truth'' is given by the scores a reference-free metric returns in a reference-based setup. The reference is computed with Google Translate. Including this factor with an additional regressor improves the $R^2$ score. 
    \item Each metric captures semantic similarity and lexical overlap to some extend. Syntactic and morphological similarity are either captured to a smaller extend or are even negatively correlated with the metric score. Especially, MoverScore and BERTScore put a high emphasis on the lexical score.
    \item For the simpler sentences of the STS dataset, the scores can be explained to a larger extend (higher $R^2$) than for WMT. This is attributed to the inhomogenity of WMT and the fact that the WMT sentences contain erroneous sentences. 
    \item Based on the finding that the metrics favour lexical overlap, \citet{kaster-2021} explore their robustness towards adversarial examples that preserve lexical overlap but change meaning. They show that permutations that have a high lexical overlap but don't preserve semantics tend to achieve better scores than permutations that preserve semantics but have a low lexical overlap. 
    \item In another experiment \citet{kaster-2021} show that the ensembling of metrics with different lexical properties can improve their overall corellation with human judgements.
\end{itemize}

In terms of the dimensions introduced in section \ref{sec:dimensions}, we can further categorize this explainability technique as ``explanation by simplification'', as a simple linear model is learned that explains the complex metric score as a linear combination of scores that can be easier understood. It is to note however, that SYM, which is determined by humans, and MOR, which is based on word embeddings, could be considered black box settings themselves. Likewise, the additional CLB criterion which leverages the explained metric itself, is also a black box. Future work might explore the dependence of the different scores. For example, by explaining SYM in terms of LEX, SYN and MOR. 

\subsection{Peturbation Checklists}
\label{sec:pertChecklist}
\citet{sai-2021} propose perturbation checklists that evaluate how susceptible metrics are towards predefined types of permutations. This allows developers to check whether all invariances that are required for a specific task are fulfilled. They start their work with the consideration that, depending on the task, sentence-level scores can describe multiple properties such as fluency, adequacy, coherence, etc. and it often is unclear, which of them are expressed in single metric scores. By using existing datasets, they show the correlation between different properties. For MT they reason that the two applicable criteria adequacy and fluency are correlated enough to use single human annotated scores. In other tasks, they diverge more, such that these should not use metrics that assign a single score. To evaluate each metric with respect to different properties, they follow \citet{ribeiro-2020} and check, how a metric behaves when property specific changes are applied to the input. Furthermore, they compare the change in the metric's score with the change in score a human would assign after the perturbation. Thus, they compute a performance score of the metric using:
$$s_c^t(e)=(h(\hat{p}_c^t)-h(p)) - f_e(\hat{p}_c^t)-f_e(p))$$
Here $s$ denotes the score for a perturbation template $t$ that applies criterion (property) $c$. $e$ denotes the metric that is explained, $h$ denotes the human score and $f_e$ denotes the score achieved by $e$. Finally, $p$ is the original model output and $\hat{p}_c^t$ the permuted output. They annotate $h$ using 15 annotators that determine on a scale from 0 to 10 how much a score should change for a perturbation. In total, they provide 34 perturbation templates.

In a first coarse evaluation \citep{sai-2021} find that most metrics have weak correlations to property specific human judgments. They note that metrics that incorporate pre-training and fine-tuning steps, such as BLEURT, would perform best. In a second evaluation step, they apply the formula described above and use perturbation templates. Here, they report the following key findings:
\begin{itemize}
    \item While the coarse evaluation already has shown shortcomings of the metrics, the fine-grained evaluation can show further problems. For example, BERTScore, BLEURT and Moverscore are shown to have problems to correctly predict the score with antonyms and negations. 
    
    We believe that this is caused by antonyms generally occurring in the same contexts as the original word \citep[e.g.][]{samenko-2021}.  E.g. "A sad cat" might be more similar in context to "A happy cat" than to "A boring cat".
    \item Metrics are unable to capture task specific properties. For example, they find that the metric ViLBERTScore for image captioning is not prone to perturbations of gender.
    \item The perturbation checklists allow to pick metrics that are strong with respect to specific properties. E.g. Moverscore would capture fluency better than BERTScore due to its ability to cope with the jumbling of words.
\end{itemize}

Following the definitions in section \ref{sec:dimensions}, the perturbation checklists are model-agnostic and can improve on all three goals. They can detect biases and model shortcomings by applying respective perturbation templates. Further, they might improve accessibility in terms of improving the understanding what a metric does. However, as it is a global technique, it doesn't support users in understanding single decisions.

==> legacy/old_structure/6_data.tex <==
\section{Datasets}
\label{datasets}
This section describes common desiderata for explainability datasets and specifics for explainable MT evaluation. Afterwards, we summarize different datasets of this domain. 
\subsection{Desiderata and Methodology}
To introduce common desiderata of datasets for explainable NLP, we summarize a recent work by \citet{wiegreffe-2021}. They give an overview of datasets for the evaluation of explainability methods for NLG in general. These datasets are comprised of human explanations for a given task. Hence, when machine learning systems are explained with an explainability technique, the human explanations can be used as a ground truth. They differentiate the datasets based on three explanation types: \textit{Highlights} (or rationales), \textit{free-text} explanations and \textit{structured explanations}. In terms of the terminology introduced in section \ref{terminology}, highlights are feature importance explanations for which the most important tokens are selected as an explanation. Further, free-text explanations were referred to as textual explanations. They define structured explanations as textual explanations that place a constraint on the form of the text in a textual explanation. 
Notably, they don't report any prior dataset in the domain of explainable MT evaluation. With SCAT \citep{yin-2021}, there is one dataset for document level machine translations, where annotators selected words that helped to disambiguate sentences with pronoun anaphora resolution and word sense disambiguation in English to French translations. For each explanation type, \citet{wiegreffe-2021} define desiderata for the data collection process:

\begin{itemize}
\item \textbf{Highlights} can fulfill three conditions: \textit{compactness}, \textit{sufficiency} and \textit{comprehensiveness}. Compactness specifies that the highlights should be short. Sufficiency specifies that the highlights alone lead to the same prediction as the original input. Finally, comprehensiveness specifies that all tokens that are important to a prediction are highlighted. The first two properties are necessary in order to test for plausibility. I.e. when humans annotate compact and sufficient highlights, the overlap with automatic explanations can be computed. Comprehensiveness is a property that is necessary for faithful explanations. Here the authors show that  the comprehensiveness of human annotations can affect plausibility evaluation. I.e. when faithful (sufficient and comprehensive) explanations of a model are generated, but the human annotated data for the plausibility evaluation is only sufficient, there is a mismatch. More comprehensive explanations might receive a lower correlation. They recommend to require high sufficiency for all highlights and high comprehensiveness for evaluations where explanations were modelled to be comprehensive. Further, post-hoc annotations of comprehensiveness should be avoided.
\item \textbf{Free-Text Explanations} are often error-prone due to their high expressivity. When they are collected, it should first be observed how humans address the task. If they address it in a certain schema, \textbf{Structured Explanations} should be used. 
\item The collection process of the explanations should be precisely reported. 
\item Not all properties of collected data are always necessary (e.g. comprehensiveness). For each property, it should be stated, which modeling- and evaluation- assumptions it causes. 
\end{itemize}


Additionally, \citet{wiegreffe-2021} propose collection strategies to increase explanation quality and diversity. To increase the quality, they propose to use \textit{Collect-And-Edit} strategies, where annotators are presented with precollected explanations and are prompted to correct them. Further, the annotators should be taught and tested on the task before starting the process. Also, binary labels should be avoided to allow ambiguous decisions. To increase the diversity, a larger number of annotators could be used for each instance. 

In terms of Machine Translation evaluation, word-level translation errors offer a good target for human explanations (see section \ref{eval4nlpdata}). This type of rationale additionally favours the sufficient and comprehensive selection, as in many cases the concept of an error is clealy defined.

\subsection{Data of the Eval4NLP 2021 shared task}
\label{eval4nlpdata}
The Eval4NLP 2021 shared task \citep{fomicheva-2021} provides the first dataset that jointly annotates sentence-level scores with word-level error highlighting in source and hypothesis of a machine translation setting. Their data comprises the language pairs et-en (Estonian-English), ro-en (Romanian-English), ru-de (Russian-German) and zh-de (Chinese-German). Source sentences from Wikipedia were translated with SOTA translation models\footnote{de-zh was translated with Google translate. The source sentences from other language pairs were translated with mBART50 \citep{tang-2020}.} to obtain the machine translations. The sentence-level scores were annotated with direct assessment \citep{graham-2016} and indicate translation quality on a scale from 1 to 100. The word-level error annotation assigns binary labels to every word that indicate whether it is an error, or not. Words missing in the translation can be highlighted in the source and words that were added wrongly in a translation, can be highlighted in the translation. The annotations were performed by multiple annotators with Cohen's Kappa inter-annotator agreement of 0.42 to 0.67 on word-level. The highest average sentence-level scores were achieved for de-zh, the lowest by ru-de.

Compared to the annotation process of MLQE-PE (see section \ref{MLQE-PE}), this has the benefit that no extra steps such as the translation error rate between post-edit and hypothesis are required. The organizers show that the number of word-level errors is indeed lower for their annotation scheme.

ToDo: show how some of the best practices described in the previous section were applied here.

\subsection{MLQE-PE}
\label{MLQE-PE}
The MLQE-PE corpus \citep{fomicheva-2020} contains sources, machine translations, human annotated direct assessment (DA) scores for translation quality and human annotated minimal post-edits (PE). The post-edits correct machine translations with as little operations as possible and are used as a basis to provide human translation error rate (HTER) scores that quantify this editing effort. Further, the corpus contains word-level error annotations of the hypotheses that are computed by comparing them with the post-edits. To obtain word-level scores for the sources, the hypotheses are aligned to the sources using fast-align \citep{dyer-2013}.

==> legacy/old_structure/7_discussion.tex <==
\section{Discussion}
\begin{itemize}
    \item Connection robustness and explainability. Hypothesis: Robustness tests are explainability techniques.
    \item Connection to word embeddings of word embedding methods and attention based methods.
\end{itemize}

Goals:
Social bias check -> Perturbation Checklists
Diagnose and Improve -> Adv Attacks (?)
Researcher Trust -> Global Regression
More expressive and accessible metrics -> Eval4NLP


==> legacy/old_structure/8_relatedWork.tex <==
\section{Related Work}
The difficulty of understanding machine learning models has implications on their real world usage. For example, it is dangerous to employ black-box systems in safety critical applications \citep{rudin-2019}. Also, they might unknowingly incorporate biases such as gender, racial, political or religious bias \citep{mehrabi-2021}. In their general data protection regulation, the European Union even requires that decisions that impact a person can be explained \citep{goodman-2017}. 
Hence, the interpretability and explainability of machine translation models forms a gateway to their broader usage (we will define these terms in the next section)\PL{Isn't it too late to introduce new things in the future work section?}. Further propelled by recent challenges, such as the eXplainable AI challenge by \citet{gunning-2017} or the explainable ML (xML) challenge by the \citet{fico-2018}, a large body of research considers this problem. Likewise, an increasing number of surveys describe core concepts, taxonomies and techniques \citep[e.g.][]{lipton-2016, barredo-arrieta-2020, danilevsky-2020, linardatos-2021, lertvittayakumjorn-2021}. This leads to a high information density, however it can also lead to ambiguous definitions (see section \ref{terminology}).\PL{Not sure what is the point of this paragraph. It looks more suitable for the first few sections rather than last few sections.} 

In the following we refer to exemplary surveys across the field. We present selected definitions and taxonomies in section \ref{terminology}. Therefore this section only provides a rough overview. \citet{lipton-2016} lays an important ground stone, by working out common goals found in interpretability research. Further, he divides the notions of transparency and post-hoc interpretability, which is related to the definitions of explainability and interpretability that we choose in section \ref{terminology}. Additionally, he provides a small taxonomy of explainability techniques based on their output type. I.e. he differs between text explanations, visualization, local explanations and explanation by example. Another important conceptual work is presented by \citet{doshi-velez-2017}. Based on a dictionary, they provide an often used explanation of interpretability \citep[e.g.][]{guidotti-2018, du-2019}. Further, they define common goals and interpretability dimensions and introduce a taxonomy of interpretability evaluation approaches. \citet{doran-2017} survey terminology across the literature and propose a notion of explainablity that incorporates reasoning. \citet{miller-2019} connects explainability research with philosophy and psychology to incorporate knowledge on how humans communicate with each other. Thereby, he also summarizes approaches for human evaluation. Despite these conceptual works, many surveys additionally provide taxonomies that group and describe existing techniques.  For example, like \citet{lipton-2016}, \citet{biran-2017, adadi-2018, dosilovic-2018, guidotti-2018, arya-2019, carvalho-2019, gilpin-2019, barredo-arrieta-2020, bodria-2021, linardatos-2021} provide taxonomies of techniques for inherent interpretability and post-hoc explainability. Most of them also use the distinction of local vs. global explainability and model-agnostic vs. model-specific explanations. \citet{guidotti-2018, bodria-2021, linardatos-2021} employ another distinction based on the input type (images, text, tabular data). \citet{montavon-2018} provide a survey targeted at the model-specific explainability of neural networks. \citet{danilevsky-2020} provide a survey that especially targets NLP. There is also work that criticizes certain developments in the XAI domain. For example, \citet{rudin-2019} warns against the usage of black-box models and post-hoc explainability and demand the development of architectures that inherently provide explanations. \citet{bastings-2020} highlight the superiority of gradient-based feature importance techniques over attention based ones.

Another strand of research explores the evaluation of explainability. For example, \citet{deyoung-2020} provide a benchmarking suite for feature-importance explainability techniques that comprises a number of techniques to evaluate plausibility and faithfulness. \citet{bodria-2021} also provide an overview of potential evaluation techniques and apply them to a small number of explainability techniques. \citet{Lertvittayakumjorn-2019} present different human evaluation schemes for text classification settings. Further surveys that consider evaluation approaches are \citet{adadi-2018, arya-2019, miller-2019, barredo-arrieta-2020, burkart-2021, linardatos-2021}.

There are also a few surveys that touch upon the need for explainable NLG evaluation.
In their survey of NLG metrics \citet{celikyilmaz-2020} see the need for explainable evaluation metrics to spot system quality issues and to achieve a higher trust in the evaluation of NLG systems. They consider that such quality issues might be unintended biases and factual inconsistencies. \citet{sai-2020} instead propose that explainable NLG metrics should focus on providing more information than just a single score (such as fluency or adequacy). 

Note, that the discussed work is not an exhaustive list of all interpretability/explainability surveys, which would go beyond the scope of this paper. To the best of our knowledge, our work is the first to survey explainability with a focus on MT evaluation.\PL{It would be great to explain more (i) the distinction of our work and previous surveys -- what we highlighted but not found in previous work (ii) on the other hand, which previous work we mainly build upon?.}

==> legacy/old_structure/9_conclusionAndFutureWork.tex <==
\section{Future Work}
\begin{itemize}
    \item Emphasize joint evaluation with faithfulness and plausibility metrics.
    \item Use example based approaches for model training
\end{itemize}

\section{Conclusion}

==> parts/10_relatedWork.tex <==
\section{Related Work} \label{sec:relatedwork}
The difficulty of understanding machine learning models has implications on their real world usage. For example, it is dangerous to employ black-box systems in safety critical applications \citep{rudin-2019}. Also, they might unknowingly incorporate biases such as gender, racial, political or religious bias \citep{mehrabi-2021}. In their general data protection regulation, the European Union even requires that decisions that impact a person can be explained \citep{goodman-2017}. 
Hence, the interpretability and explainability of machine translation models forms a gateway to their broader usage (we will define these terms in the next section)\PL{Isn't it too late to introduce new things in the future work section?}. Further propelled by recent challenges, such as the eXplainable AI challenge by \citet{gunning-2017} or the explainable ML (xML) challenge by the \citet{fico-2018}, a large body of research considers this problem. Likewise, an increasing number of surveys describe core concepts, taxonomies and techniques \citep[e.g.][]{lipton-2016, barredo-arrieta-2020, danilevsky-2020, linardatos-2021, lertvittayakumjorn-2021}. This leads to a high information density, however it can also lead to ambiguous definitions (see section \ref{sec:xai}).\PL{Not sure what is the point of this paragraph. It looks more suitable for the first few sections rather than last few sections.} 

In the following we refer to exemplary surveys across the field. We present selected definitions and taxonomies in sections \ref{sec:xai} and \ref{sec:taxonomy}. Therefore this section only provides a rough overview. \citet{lipton-2016} lays an important ground stone, by working out common goals found in interpretability research. Further, he divides the notions of transparency and post-hoc interpretability, which is related to the definitions of explainability and interpretability that we choose in section \ref{sec:xai}. Additionally, he provides a small taxonomy of explainability techniques based on their output type. I.e. he differs between text explanations, visualization, local explanations and explanation by example. Another important conceptual work is presented by \citet{doshi-velez-2017}. Based on a dictionary, they provide an often used explanation of interpretability \citep[e.g.][]{guidotti-2018, du-2019}. Further, they define common goals and interpretability dimensions and introduce a taxonomy of interpretability evaluation approaches. \citet{doran-2017} survey terminology across the literature and propose a notion of explainablity that incorporates reasoning. \citet{miller-2019} connects explainability research with philosophy and psychology to incorporate knowledge on how humans communicate with each other. Thereby, he also summarizes approaches for human evaluation. Despite these conceptual works, many surveys additionally provide taxonomies that group and describe existing techniques.  For example, like \citet{lipton-2016}, \citet{biran-2017, adadi-2018, dosilovic-2018, guidotti-2018, arya-2019, carvalho-2019, gilpin-2019, barredo-arrieta-2020, bodria-2021, linardatos-2021} provide taxonomies of techniques for inherent interpretability and post-hoc explainability. Most of them also use the distinction of local vs. global explainability and model-agnostic vs. model-specific explanations. \citet{guidotti-2018, bodria-2021, linardatos-2021} employ another distinction based on the input type (images, text, tabular data). \citet{montavon-2018} provide a survey targeted at the model-specific explainability of neural networks. \citet{danilevsky-2020} provide a survey that especially targets NLP. There is also work that criticizes certain developments in the XAI domain. For example, \citet{rudin-2019} warns against the usage of black-box models and post-hoc explainability and demand the development of architectures that inherently provide explanations. \citet{bastings-2020} highlight the superiority of gradient-based feature importance techniques over attention based ones.

Another strand of research explores the evaluation of explainability. For example, \citet{deyoung-2020} provide a benchmarking suite for feature-importance explainability techniques that comprises a number of techniques to evaluate plausibility and faithfulness. \citet{bodria-2021} also provide an overview of potential evaluation techniques and apply them to a small number of explainability techniques. \citet{Lertvittayakumjorn-2019} present different human evaluation schemes for text classification settings. Further surveys that consider evaluation approaches are \citet{adadi-2018, arya-2019, miller-2019, barredo-arrieta-2020, burkart-2021, linardatos-2021}.

There are also a few surveys that touch upon the need for explainable NLG evaluation.
In their survey of NLG metrics, \citet{celikyilmaz-2020} see the need for explainable evaluation metrics to spot system quality issues and to achieve a higher trust in the evaluation of NLG systems. They consider that such quality issues might be unintended biases and factual inconsistencies. \citet{sai-2020} instead propose that explainable NLG metrics should focus on providing more information than just a single score (such as fluency or adequacy). 

Note, that the discussed work is not an exhaustive list of all interpretability/explainability surveys, which would go beyond the scope of this paper. To the best of our knowledge, our work is the first to survey explainability with a focus on MT evaluation.\PL{It would be great to explain more (i) the distinction of our work and previous surveys -- what we highlighted but not found in previous work (ii) on the other hand, which previous work we mainly build upon?.}

==> parts/5_data.tex <==
\section{Datasets}\label{sec:datasets} %\todo{SE: maybe this section should have a different location}
% 
\label{sec:datasets}
Datasets play an important role in evaluation.
In this section, we first describe the desired properties of 
explainability datasets in general, and then review 
existing explainable MT evaluation datasets and discuss their properties.

\subsection{Explainability Datasets: Methods and Desiderata }
Explainability datasets usually include human explanations for a certain task
(e.g., text classification).
When machine learning systems for the task are explained with 
an explainability technique, the machine generated explanations
can be compared against the human ground truths to measure
their plausibility. 
As included in \citet{wiegreffe-2021}, 
%
three types of explanations \PL{three types of human ground truths?} are widely recognized:
\textit{Highlights} (also known as rationales), \textit{free-text} explanations 
and \textit{structured explanations}. 
%
Based on the terminology we introduced in Section \ref{sec:xai}, 
highlights are \emph{feature importance explanations}, where 
the most important tokens are selected as an explanation. 
Free-text explanations and structured explanations are
both \emph{textual explanations}, but structured explanations have constraints
on the form of the text. 

%YG: unclear how the following part is connected other parts, hence deleted
%Notably, they don't report any prior dataset in the domain of explainable MT evaluation. With SCAT \citep{yin-2021}, there is one dataset for document level machine translations, where annotators selected words that helped to disambiguate sentences with pronoun anaphora resolution and word sense disambiguation in English to French translations. 

\paragraph{Desired Properties}
Each explanation type has some unique desiderata \cite{wiegreffe-2021}.
%
For \emph{highlights}, %they have three desired properties:
these include: 
\emph{compactness}, \emph{sufficiency} and \emph{comprehensiveness}.
Compactness requires the highlighted parts to be short; 
sufficiency means the highlights alone should lead to the same 
prediction as the original input;
comprehensiveness means all important tokens should be highlighted.
%
\emph{Compactness} and \emph{sufficiency} are necessary for testing 
\emph{plausibility} (definition in Section \ref{sec:xai}): 
if the human explanations are compact and sufficient,
the plausibility of the machine generated explanations can 
be measured by their overlap with the human explanations. \PL{We should state clearly that comprehensiveness and sufficiency are from machine's viewpoint or humans' viewpoint. These terms in the literature consider them from the machine's viewpoint; however, can they be desired properties of datasets created by humans then? --> \CL good question. I think in their paper it describes a property of the explanation, be it of the humans annotating or the machine generating. }
%
%Comprehensiveness guarantees the \emph{faithfulness} of the 
%human explanations and it also affects plausibility evaluation. 
\PL{Not sure whether comprehensiveness guarantees faithfulness. -->\\CL: I guess I meant faithful from a human perspective. E.g. it is a complete answer that is given with nothing left out, that should also be reproducible. But yes, it is not a good idea to use the terminology like that. I think we might want to drop the wiegreffe part anyways.} 
%YG: the following part is confusing, involving too many terminology
%I.e. when faithful (sufficient and comprehensive) explanations of a model are generated, but the human annotated data for the plausibility evaluation is only sufficient, there is a mismatch. More comprehensive explanations might receive a lower correlation. They recommend to require high sufficiency for all highlights and high comprehensiveness for evaluations where explanations were modelled to be comprehensive. Further, post-hoc annotations of comprehensiveness should be avoided.
\todo{YG: any desired properties for the other types of explanations?}
In terms of Machine Translation evaluation, word-level 
translation errors can naturally be used as highlight explanations
(see Section \ref{eval4nlpdata});
sufficiency and comprehensiveness are particularly desirable
for these explanations, because in many cases the concept 
of error types are clearly defined (and hence the compactness is enforced).
\todo{YG: check whether this is right.}


Note that not all aforementioned desired properties are always 
necessary (e.g., comprehensiveness). For each property, 
it should be stated which modeling and evaluation assumptions 
the property requires. 

\paragraph{Data Collection}
To elicit high quality human explanations, some recommended
practices have been identified \cite{wiegreffe-2021}.
%
As a general rule, the collection process of the explanations 
should be precisely reported. 
To increase the quality, the \textit{Collect-And-Edit} strategy
can be used, where annotators are presented with precollected 
explanations and are prompted to correct them. 
Further, the annotators should be taught and tested on the task 
before starting the process. 
 \PL{But many papers ask humans to highlight important tokens which are turned into binary labels? \\--> CL: yes I removed the sentence. It was about the outcome that is explained, i.e. the human label of the main task. For MT it is usually diverse enough with at least 5-point scales.}
%
To increase the diversity, a larger number of annotators could 
be used for each instance. 
%
For free-text explanations, they are often error-prone due to high expressively; 
hence, to reduce errors,  it should first be observed how humans address the task. 
If they address it in a certain schema, \textbf{Structured Explanations} should be used. % 
\PL{Can we add citations of papers using each of the recommended practices?}


\subsection{Datasets}
\label{eval4nlpdata}

%In this section 
We now review datasets that can be leveraged in the context of explainable MT evaluation and discuss to which degree they fulfill the previous desiderata.

\paragraph{Human annotated highlights}
Few datasets employ human annotated rationales as explanations for machine translation evaluation.
The Eval4NLP 2021 shared task \citep{fomicheva-2021}
%aimed at xxx. It
provided the first dataset that jointly annotated 
sentence-level scores with word-level error highlights (seen as explanations for the sentence-level scores) for the MT setting.
Word-level highlights were annotated in both the input
text and the candidate translations.
%
Their data comprises the language pairs et-en (Estonian-English), 
ro-en (Romanian-English), ru-de (Russian-German) and 
zh-de (Chinese-German). Source sentences from Wikipedia 
were translated with SOTA translation 
models.\footnote{de-zh was translated with 
Google translate. The other language pairs were translated with mBART50 \citep{tang-2020}.}
The sentence-level scores were annotated with direct 
assessment \citep{graham-2016} and they indicate the 
translation quality on a scale from 1 to 100. 
%
The word-level error annotations are binary labels
for each token indicating whether it is an error or not.
For missing words in the translation, their corresponding
words in the source were highlighted. 
Wrongly added words in translations are also highlighted.
%
The annotations were performed by multiple annotators with Cohen's Kappa inter-annotator agreement of 0.42 to 0.67 on word-level. %The highest average sentence-level scores were achieved for de-zh, and the lowest were by ru-de.

%Another dataset which employs a similar annotation scheme in the domain of crosslingual divergence: https://aclanthology.org/2020.emnlp-main.121.pdf


\paragraph{Automatically annotated highlights}
In the domain of quality estimation, various datasets have been created that consist of automatically labeled word-level errors, e.g. on the basis of HTER \citep{snover-2006}.
The MLQE-PE corpus \citep{fomicheva-2020} contains sources, 
machine translations, human annotated direct assessment (DA) 
scores for translation quality, and human annotated post-edits (PEs). 
The PEs correct machine translations with 
minimal number of operations.
%they are used as a basis to provide 
%human translation error rate (HTER) scores that quantify this editing effort. 
Word-level error scores were also provided in the corpus, 
which were computed by measuring the misalignments 
between the translations and the inputs using fast-align \citep{dyer-2013}.
%
With the error scores, incorrect tokens in the translations 
can be easily identified, which in turn can be used as (explanation) highlights.

\paragraph{MQM Datasets} \item \textbf{MQM:} \label{MQM} MQM (Multidimensional Quality Metrics) is an annotation method in which multilingual annotators assign fine grained error labels to translations \citep{lommel-2014, lommel-2015}. In a recent evaluation, \citet{freitag-2021} compare direct assessment \citep{graham-2015} and MQM. They label English-German and Chinese-English datasets with an MQM annotation scheme. The scheme uses main categories such as accuracy, fluency, style and terminology as well as several subcategories. Errors can be major, minor or neutral. A sentence score is inferred by computing the sum of differently weighted errors (and averaging them). The authors find that DA scores do not correlate well with MQM scores. Additionally, they find that MQM scores can distinguish human translations better from machine translations than DA scores (by ranking translations based on the scores). As MQM's phrase-level error annotations suffer from weak inter-annotator agreement \citep{}, they are usually aggregated to sentence-level scores \citep{}. Still, following the considerations of Section \ref{}, MQM annotations themselves can be interpreted as explanations, as they provide a fine-grained description of the errors in a translation. 

\textcolor{red}{TODO: how many desired properties do these two datasets have? which
annotation practice they have followed? We need to connect two subsections!}

%\textcolor{red}{Compared to the annotation process of MLQE-PE (see section \ref{MLQE-PE}), this has the benefit that no extra steps such as the translation error rate between post-edit and hypothesis are required. The organizers show that the number of word-level errors is indeed lower for their annotation scheme.}

%\textcolor{red}{MF: Discuss how this is different from a) OK/BAD <- HTER b) MQM}

%ToDo: show how some of the best practices described in the previous section were applied here.


==> parts/9_discussion.tex <==
\section{Discussion} \label{sec:discussion}
\begin{itemize}
    \item Connection robustness and explainability. Hypothesis: Robustness tests are explainability techniques.
    \item Connection to word embeddings of word embedding methods and attention based methods.
\end{itemize}

Goals:
Social bias check -> Perturbation Checklists
Diagnose and Improve -> Adv Attacks (?)
Researcher Trust -> Global Regression
More expressive and accessible metrics -> Eval4NLP


==> parts/old_6_data.tex <==
\section{Datasets}\todo{SE: maybe this section should have a different location}
% \label{datasets}
\label{sec:datasets}
Some papers use specifically collected datasets to evaluate explainability approaches.
This section describes common desiderata for explainability datasets and specifics for explainable MT evaluation. Afterwards, we summarize different datasets of this domain. 
\subsection{Desiderata and Methodology}
To introduce common desiderata of datasets for explainable NLP, we summarize a recent work by \citet{wiegreffe-2021}. They give an overview of datasets for the evaluation of explainability methods for NLG in general. These datasets are comprised of human explanations for a given task. Hence, when machine learning systems are explained with an explainability technique, the human explanations can be used as a ground truth. They differentiate the datasets based on three explanation types: \textit{Highlights} (or rationales), \textit{free-text} explanations and \textit{structured explanations}. In terms of the terminology introduced in section \ref{sec:xai}, highlights are feature importance explanations for which the most important tokens are selected as an explanation. Further, free-text explanations were referred to as textual explanations. They define structured explanations as textual explanations that place a constraint on the form of the text in a textual explanation. 
Notably, they don't report any prior dataset in the domain of explainable MT evaluation. With SCAT \citep{yin-2021}, there is one dataset for document level machine translations, where annotators selected words that helped to disambiguate sentences with pronoun anaphora resolution and word sense disambiguation in English to French translations. For each explanation type, \citet{wiegreffe-2021} define desiderata for the data collection process:

\begin{itemize}
\item \textbf{Highlights} can fulfill three conditions: \textit{compactness}, \textit{sufficiency} and \textit{comprehensiveness}. Compactness specifies that the highlights should be short. Sufficiency specifies that the highlights alone lead to the same prediction as the original input. Finally, comprehensiveness specifies that all tokens that are important to a prediction are highlighted. The first two properties are necessary in order to test for plausibility. I.e. when humans annotate compact and sufficient highlights, the overlap with automatic explanations can be computed. Comprehensiveness is a property that is necessary for faithful explanations. Here the authors show that  the comprehensiveness of human annotations can affect plausibility evaluation. I.e. when faithful (sufficient and comprehensive) explanations of a model are generated, but the human annotated data for the plausibility evaluation is only sufficient, there is a mismatch. More comprehensive explanations might receive a lower correlation. They recommend to require high sufficiency for all highlights and high comprehensiveness for evaluations where explanations were modelled to be comprehensive. Further, post-hoc annotations of comprehensiveness should be avoided.
\item \textbf{Free-Text Explanations} are often error-prone due to their high expressivity. When they are collected, it should first be observed how humans address the task. If they address it in a certain schema, \textbf{Structured Explanations} should be used. 
\item The collection process of the explanations should be precisely reported. 
\item Not all properties of collected data are always necessary (e.g. comprehensiveness). For each property, it should be stated, which modeling- and evaluation- assumptions it causes. 
\end{itemize}


Additionally, \citet{wiegreffe-2021} propose collection strategies to increase explanation quality and diversity. To increase the quality, they propose to use \textit{Collect-And-Edit} strategies, where annotators are presented with precollected explanations and are prompted to correct them. Further, the annotators should be taught and tested on the task before starting the process. Also, binary labels should be avoided to allow ambiguous decisions. To increase the diversity, a larger number of annotators could be used for each instance. 

In terms of Machine Translation evaluation, word-level translation errors offer a good target for human explanations (see section \ref{eval4nlpdata}). This type of rationale additionally favours the sufficient and comprehensive selection, as in many cases the concept of an error is clealy defined.

\subsection{Data of the Eval4NLP 2021 shared task}
\label{eval4nlpdata}
The Eval4NLP 2021 shared task \citep{fomicheva-2021} provides the first dataset that jointly annotates sentence-level scores with word-level error highlighting in source and hypothesis of a machine translation setting. Their data comprises the language pairs et-en (Estonian-English), ro-en (Romanian-English), ru-de (Russian-German) and zh-de (Chinese-German). Source sentences from Wikipedia were translated with SOTA translation models\footnote{de-zh was translated with Google translate. The source sentences from other language pairs were translated with mBART50 \citep{tang-2020}.} to obtain the machine translations. The sentence-level scores were annotated with direct assessment \citep{graham-2016} and indicate translation quality on a scale from 1 to 100. The word-level error annotation assigns binary labels to every word that indicate whether it is an error, or not. Words missing in the translation can be highlighted in the source and words that were added wrongly in a translation, can be highlighted in the translation. The annotations were performed by multiple annotators with Cohen's Kappa inter-annotator agreement of 0.42 to 0.67 on word-level. The highest average sentence-level scores were achieved for de-zh, the lowest by ru-de.

\textcolor{red}{Compared to the annotation process of MLQE-PE (see section \ref{MLQE-PE}), this has the benefit that no extra steps such as the translation error rate between post-edit and hypothesis are required. The organizers show that the number of word-level errors is indeed lower for their annotation scheme.}

\textcolor{red}{MF: Discuss how this is different from a) OK/BAD <- HTER b) MQM}

ToDo: show how some of the best practices described in the previous section were applied here.

\subsection{MLQE-PE}
\label{MLQE-PE}
The MLQE-PE corpus \citep{fomicheva-2020} contains sources, machine translations, human annotated direct assessment (DA) scores for translation quality and human annotated minimal post-edits (PE). The post-edits correct machine translations with as little operations as possible and are used as a basis to provide human translation error rate (HTER) scores that quantify this editing effort. Further, the corpus contains word-level error annotations of the hypotheses that are computed by comparing them with the post-edits. To obtain word-level scores for the sources, the hypotheses are aligned to the sources using fast-align \citep{dyer-2013}.

==> tables/local.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l}
         \toprule
         Kõik \textcolor{blue}{rahvaülikooli} loengud salvestati \textcolor{blue}{magnetofonilindile} . \\
         All the lectures from the \attacked{national} \attacked{university} were recorded on a \attacked{magnet} \attacked{contributor} . \\
         \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{lll}
         \toprule
         ref & Jane loves Joe \\
         hyp & It is Joe that Jane adores \\
         hyp-adv & Joe loves Jane \\ \midrule
         \multicolumn{2}{c}{$\mathfrak{m}(\text{ref},\text{hyp}) \overset{?}{\gtrless} \mathfrak{m}(\text{ref},\text{hyp-adv})$}\\
         \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{ccccccc}
        \toprule
         %\pbox{123451} & & \pbox{1} & & \pbox{11} & & \pbox{1111}  \\
         \mybox{.5cm}{1.5cm} & & \mybox[blue]{.5cm}{0.5cm} && 
         \mybox[red]{.5cm}{0.3cm} &&
         \mybox[brown]{.5cm}{0.7cm}\\
         metric score & $=$ & semantics & $+$ & syntax & $+$ & lexical overlap 
         \\
         \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}
\parbox{.45\linewidth}{
    \centering
    \begin{tabular}{lll}
         \toprule
         ref & Jane loves Joe \\
         hyp & It is Joe that Jane adores \\
         hyp-adv & Joe loves Jane \\ \midrule
         \multicolumn{2}{c}{$\mathfrak{m}(\text{ref},\text{hyp}) \overset{?}{\gtrless} \mathfrak{m}(\text{ref},\text{hyp-adv})$}\\
         \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
}
\hfill
\parbox{.45\linewidth}{
    \centering
    \begin{tabular}{ccccccc}
        \toprule
         %\pbox{123451} & & \pbox{1} & & \pbox{11} & & \pbox{1111}  \\
         \mybox{.5cm}{1.5cm} & & \mybox[blue]{.5cm}{0.5cm} && 
         \mybox[red]{.5cm}{0.3cm} &&
         \mybox[brown]{.5cm}{0.7cm}\\
         metric score & $=$ & semantics & $+$ & syntax & $+$ & lexical overlap 
         \\
         \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
}
\end{table}

==> tables/metric_typology_v1.tex <==
\begin{table}[!htb]
\centering
%\begin{tabular}{c|cccc}
    \begin{tabularx}{\textwidth}{lXX}
     \toprule
     \textbf{Dimension} &  \textbf{Description} & \textbf{Selected Examples} \\ 
     \midrule
     \emph{Degree of automation} & Whether evaluation metrics are automatic & Most metrics  \\ \hline
     \emph{Use of embeddings} & Whether metrics take semantics into account & MoverScore (+), BERTScore (+), BARTScore (+), BLEU (-)\\ \hline 
     \emph{Supervision} & The degree of supervision a metric requires \\
     Training & & BLEURT (+), COMET (+), BERTScore (-)\\
     Use of references & & COMET (+), BARTScore (+), XMoverScore (-)\\ \hline
     \emph{Metric task} & How the metric is induced & \\ 
     Unsupervised Matching & & MoverScore, BERTScore\\
     Supervised regression/ranking & & TransQuest, COMET\\
     Text generation & & PRISM, BARTScore\\
     Question answering & & QAEval\\
     \bottomrule
\end{tabularx}
\caption{A typology of categorizations for evaluation metrics.}
\label{table:metrics}
\end{table}


==> tables/metric_typology_v2.tex <==
\begin{table}[!htb]
\centering
%\begin{tabular}{c|cccc}
    \begin{tabularx}{\textwidth}{lXX}
     \toprule
     \textbf{Dimension} &  \textbf{Description} \\ 
     \midrule
     \emph{Type of input} & Whether source, reference translation or both are used as benchmark for comparison \\ \hline
     \emph{Input representation} & Whether the metric relies on words or uses a continuous representation of the input such as word embeddings \\ \hline 
     \emph{Supervision} & Whether the metrics is deterministic or requires some form of learning \\ \hline
     \emph{Granularity} & Word-level, sentence-level, document-level or system-level \\ \hline
     \emph{Quality aspect} & Fluency, adequacy, etc. \\ \hline
     \emph{Learning objective} & Regression, ranking, etc. \\ \hline
     \emph{Interpretability} & Whether the metric's output is interpretable \\
     \bottomrule
\end{tabularx}
\caption{A typology of categorizations for evaluation metrics.}
\label{table:metrics}
\end{table}

